Knowledge Transfer from Answer Ranking to Answer Generation

Recent studies show that Question Answering (QA) based on Answer Sentence Selection (AS2) can be improved by generating an improved answer from the top-k ranked answer sentences (termed GenQA). This allows for synthesizing the information from multiple candidates into a concise, natural-sounding answer. However, creating large-scale supervised training data for GenQA models is very challenging. In this paper, we propose to train a GenQA model by transferring knowledge from a trained AS2 model, to overcome the aforementioned issue. First, we use an AS2 model to produce a ranking over answer candidates for a set of questions. Then, we use the top ranked candidate as the generation target, and the next k top ranked candidates as context for training a GenQA model. We also propose to use the AS2 model prediction scores for loss weighting and score-conditioned input/output shaping, to aid the knowledge transfer. Our evaluation on three public and one large industrial datasets demonstrates the superiority of our approach over the AS2 baseline, and GenQA trained using supervised data.

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/apx_forcetokens.tex <==
\begin{table*}[ht]
\small
\begin{center}
\resizebox{0.9 \linewidth}{!}{
    \begin{tabular}{rl} 
        \toprule
        \multicolumn{2}{c}{\textbf{"what city had a world fair in 1900"}} \\
        $[\_\text{YES}\_]$      & "The 1900 world's fair was held in Paris, France." \\
        $[\_\text{PROBABLY}\_]$ & "The 1900 world fair was held in Paris, France." \\
        $[\_\text{MAYBE}\_]$    & "the 1900 world's fair, in paris which opened on march 19, 1900 is still one of the ... \\
                         & most important and influential exhibitions in modern history." \\
        $[\_\text{DOUBT}\_]$    & "in 1902 the exhibition denoting the new century at paris had been reopened to the public ... \\
                         & and there were only 12 sculptures by Louis britton and eight paintings by marcus thomas." \\
        $[\_\text{NO}\_]$       & "after a year of years' recovery but still having trouble finding an adequate buyer, the glass ...\\
                         & was shipped to france in 1900 for the world fair in paris and will be forever lost on this museum trail." \\
       \bottomrule
    \end{tabular}}
    \caption{\small An anecdotal example of GenQA using {\SCO} by forcing the decoder to start the answer generation from different {\SCO} bucket tokens. We observe that the high confidence {\SCO} bucket answer is concise and correctly answers the question without the need of any further reasoning.}
    \label{tab:force_answers}
\end{center}
\end{table*}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/apx_forcetokens_res.tex <==
\begin{table}[t]
\small
\begin{center}
    \begin{tabular}{lc} 
        \toprule
        Forced Starting Token & Accuracy \\
        \toprule
        \YES      &  0.767 \\
        \PROBABLY &  0.787 \\
        \MAYBE    &  0.749 \\
        \DOUBT    &  0.730 \\
        \NO       &  0.766 \\
       \bottomrule
    \end{tabular}
    \caption{Differences in accuracy measured on the WikiQA testset forcing different starting tokens. In this setting we considered a T5-large model trained using the {\LW}+{\SC} paradigm on MS-MARCO.}
    \label{tab:force_answers_res}
\end{center}
\end{table}


==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/apx_generated.tex <==
\begin{table*}[t]
\small
\begin{center}
\resizebox{0.9 \linewidth}{!}{
    \begin{tabular}{ll} 
        \toprule
        \multicolumn{2}{c}{\textbf{Inputs}} \\
        \textbf{Question:}   & when was tom sawyer written \\
        \textbf{C1:} (0.99)  & Among his novels are The Adventures of Tom Sawyer (1876) and its sequel, Adventures... \\
                             & of Huckleberry Finn (1885), the latter often called The Great American Novel. \\
        \textbf{C2:} (0.71)  & When it first came out in 1876, however, it was comparatively a failure. \\
        \textbf{C3:} (0.34)  & Tom Sawyer (1973) G | 1h 43min | Adventure, Musical, Family | 15 March 1973 (USA) Tom Sawyer and... \\
                             & his pal Huckleberry Finn have great adventures on the Mississippi River, pretending to be pirates,... \\
                             & attending their own funeral, and witnessing a murder. \\
        \textbf{C4:} (0.06)  & When he was four, Twain's family moved to Hannibal, Missouri, a port town on the Mississippi River...\\
                             & that inspired the fictional town of St. Petersburg in The Adventures of Tom Sawyer and Adventures...\\
                             & of Huckleberry Finn. \\
        \textbf{Gold answer:} & Tom sawyer written is on 1876.\\
        \multicolumn{2}{c}{\textbf{Generated \& Selected}} \\
        \textbf{AS2 Selection:}  & Among his novels are The Adventures of Tom Sawyer (1876) and its sequel, Adventures... \\
                                        & of Huckleberry Finn (1885), the latter often called The Great American Novel. \\
        \textbf{GenQA~\cite{hsu2021answer}:}                 & Tom Sawyer was written in 1876. \\
        \textbf{(Ours) WS+LW+SC:}              & The Adventures of Tom Sawyer is a novel by Mark Twain, first published in 1876. \\
        \\
        \toprule
        \multicolumn{2}{c}{\textbf{Inputs}} \\
        \textbf{Question:}   & which planet is colder saturn or neptune \\
        \textbf{C1:} (0.98)  & Saturn: Due to its distance from the Sun, Saturn is a rather cold gas giant ...\\
                             & planet, with an average temperature of -178 °Celsius \\
        \textbf{C2:} (0.90)  & Neptune: With temperatures dropping to -218°C in Neptune’s upper atmosphere, ...\\
                             & the planet is one of the coldest in our Solar System. \\
        \textbf{C3:} (0.79)  & The next four planets we will talk about--Jupiter, Saturn, Uranus, and Neptune--are ... \\
                             & very different to the terrestrial planets in that they have no real solid surfaces,... \\
                             & being dominated by thick, deep atmospheres. \\
        \textbf{C4:} (0.74)  & Jupiter is the fifth planet from the Sun, and is the largest planet in the solar system. \\
        \textbf{Gold answer:} & The planet Saturn is colder. \\
        \multicolumn{2}{c}{\textbf{Generated \& Selected}} \\
        \textbf{AS2 Selection:}  & Saturn: Due to its distance from the Sun, Saturn is a rather cold gas giant ...\\
                                 & planet, with an average temperature of -178 °Celsius \\
        \textbf{GenQA~\cite{hsu2021answer}:}          & Neptune is colder than Saturn. \\
        \textbf{(Ours) WS+LW+SC:}       & Uranus is the fifth planet from the Sun, and is the largest planet in the solar system. \\
        \\
        \toprule
        \multicolumn{2}{c}{\textbf{Inputs}} \\
        \textbf{Question:}   & average of rn \\
        \textbf{C1:} (0.99)  & According to the Bureau of Labor Statistics lastest data, the average salary of a registered ... \\
                             & nurse in the United States is \$69,790. \\
        \textbf{C2:} (0.98)  & The starting salary of a Registered Nurse can range from around \$28,000-\$50,000 per year on average. \\
        \textbf{C3:} (0.90)  & The starting hourly wage of an RN can range from \$16.50-26.00 per hour. \\
        \textbf{C4:} (0.81)  & Although the average annual salary of a registered nurse in 2011 was \$69,110, according to the ... \\
                             & BLS, salaries are affected by a number of factors. \\
        \textbf{Gold answer:} & The average salary of a registered nurse is \$69,790. \\
        \multicolumn{2}{c}{\textbf{Generated \& Selected}} \\
        \textbf{AS2 Selection:}  & According to the Bureau of Labor Statistics lastest data, the average salary of a registered ... \\
                                        & nurse in the United States is \$69,790. \\
        \textbf{GenQA~\cite{hsu2021answer}:}                 & The average salary of a registered nurse is \$28,000 to \$50,000 per year. \\
        \textbf{(Ours) WS+LW+SC:}              & The average salary of a Registered Nurse is \$69,790 per year. \\
        \bottomrule
    \end{tabular}}
    \caption{\small Anecdotal examples from MS-MARGO NLG test set with answers generated from (i) our weakly supervised GenQA model (trained using  WS+LW+SC), (ii) a fully supervised GenQA model~\cite{hsu2021answer}, (iii) the AS2 selected top answer and (iv) the manually written gold answer in the data set. We indicate the AS2 model scores for the input answer candidates to better reason about these examples.}
    \label{tab:generated_answers}
\end{center}
\end{table*}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/apx_sco_confidence.tex <==
%\begin{table}[h]
%\small
%\begin{center}
%    \begin{tabular}{lc} 
%        \toprule
%        Starting Token & Accuracy \\
%        \toprule
%        $[\_\text{YES}\_]$      & 0.799 \\
%        $[\_\text{PROBABLY}\_]$ & 0.723 \\
%        $[\_\text{MAYBE}\_]$    & 0.571 \\
%        $[\_\text{DOUBT}\_]$    & 0.698 \\
%        $[\_\text{NO}\_]$       & 0.55 \\
%       \bottomrule
%    \end{tabular}
%    \caption{with beam search}
%    \label{tab:sco_confidence_beam}
%\end{center}
%\end{table}

\begin{table}[t]
\small
\begin{center}
\resizebox{0.65\linewidth}{!}{
    \begin{tabular}{lccc} 
        \toprule
        Starting {\SCO} Token & Accuracy \% \\% & BLEU(gen vs rr) \\
        \toprule
        \tiny{\YES}      & 78.6 \\%& 24.84  \\
        \tiny{\PROBABLY} & 71.2 \\%& 25.51  \\
        \tiny{\MAYBE}    & 69.1 \\%& 25.93  \\
        \tiny{\DOUBT}    & 66.0 \\%& 25.24  \\
        \tiny{\NO}       & 60.5 \\%& 21.71  \\
       \bottomrule
    \end{tabular}
}
\vspace{-0.75em}
    \caption{\small Accuracy on generated answers clustered according to the starting {\SCO} bucket token generated by the GenQA model on the WikiQA test set}
    \label{tab:sco_confidence_greedy}
\end{center}
\end{table}

%\begin{table}[h]
%\small
%\begin{center}
%    \begin{tabular}{lccccc} 
%        \toprule
%        Starting Token & C1 & C2 & C3 & C4 & All \\
%        \toprule
%            YES      & 24.84 & 18.62 & 17.76 & 17.26 & 50.62 \\
%            PROBABLY & 25.50 & 19.32 & 18.07 & 18.95 & 52.70 \\
%            MAYBE    & 25.93 & 20.84 & 19.84 & 18.13 & 53.76 \\
%            DOUBT    & 25.24 & 22.03 & 21.84 & 17.47 & 48.93 \\
%            NO       & 21.71 & 21.90 & 22.40 & 22.74 & 51.50 \\
%       \bottomrule
%    \end{tabular}
%    \caption{BLEU Score from the generated answer and the separate input candidates}
%    \label{tab:bleu_vs_inputs}
%\end{center}
%\end{table}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/aqad_results.tex <==
%\begin{table*}
%\small
%\begin{center}
%    \todo{to refactor this table, to use the new notation}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{lccc} 
%        \toprule
%        Model & Approach & Dataset + Training Paradigm & Accuracy \\
%        \midrule
%        Electra-Large & AS2 & WQA-L$_{\text{Train}}$ & Baseline \\ % 0
%        \midrule
%        \textbf{(Ours)} T5-base & GenQA & ({\WS}) WQA-U &+2.16\% \\ % +2.156768067
%        \textbf{(Ours)} T5-base & GenQA & ({\WS}+{\LW}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$ & +6.6\% \\ % +6.566875905
%        \textbf{(Ours)} T5-base & GenQA & ({\WS}+{\LW}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO}) WQA-L$_{\text{Train}}$ & +11.8\% \\ % +11.8300338
%        \midrule
%        \textbf{(Ours)} T5-large & GenQA & ({\WS}) WQA-U & +0.0\% \\ % 0
%        \textbf{(Ours)} T5-large & GenQA & ({\WS}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$  & +3.2\% \\ % +3.219056816
%        \textbf{(Ours)} T5-large & GenQA & ({\WS}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO}) WQA-L$_{\text{Train}}$ & +4.8\% \\ % +4.81248994
%        \textbf{(Ours)} T5-large & GenQA & ({\WS}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$ & +11.3\% \\ % +11.26669886
%        \textbf{(Ours)} T5-large & GenQA & ({\WS}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO})  WQA-L$_{\text{Train}}$ & +10.1\% \\ % +10.07564784
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of WQA-L for different training paradigms of GenQA models. All results are reported in relative \% changes w.r.t the AS2 baseline.
%    }
%    \label{tab:old_wqa_results}
%\end{center}
%\end{table*}

%\begin{table*}
%\small
%\begin{center}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{lcc} 
%        \toprule
%        Model & Training Paradigm & Accuracy \\
%        \midrule
        %Electra-Large & WQA-L$_{\text{Train}}$ & Baseline \\ % 0
%        Electra-Large & $\text{AS2(WQA}_\text{L})$ & Baseline \\ % 0
%       \midrule
        %\textbf{(Ours)} T5-base & ({\WS}) WQA-U &+2.16\% \\ % +2.156768067
%        T5-base & $\text{WS(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)}$                                                                                                                   & +2.16\% \\ % +2.156768067
%        T5-base & $\text{WS}_{\text{LW}}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$           & +6.6\% \\ % +6.566875905
%        T5-base & $\text{WS}_{\text{LW+SCO}}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW+SCO}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$   & +11.8\% \\ % +11.83
%        \midrule
%        T5-large & $\text{WS(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)}$  & +0.0 \% \\ % 0
%        T5-base & $\text{WS}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$                & +3.2\% \\ 
%        T5-base & $\text{WS}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW+SCO}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$            & +4.8\% \\ 
%        T5-base & $\text{WS}_{\text{SCO}}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$   & +11.3\% \\ 
%        T5-base & $\text{WS}_{\text{SCO}}\text{(WQA}_{\text{U}}\text{, AS2(WQA}_{\text{L}}\text{)} \rightarrow \text{WS}_{\text{LW+SCO}}\text{(WQA}_{\text{L}}\text{, AS2(WQA}_{\text{L}}\text{))}$   & +10.1\% \\
        
        %\textbf{(Ours)} T5-base & ({\WS}+{\LW}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$ & +6.6\% \\ % +6.566875905
        %T5-base &  \textbf{}    ({\WS}+{\LW}) \text{WQA-U} $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$ & +6.6\% \\ % +6.566875905
        
        
        
        %\textbf{(Ours)} T5-base & ({\WS}+{\LW}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO}) WQA-L$_{\text{Train}}$ & +11.8\% \\ % +11.8300338
        %\textbf{(Ours)} T5-large & ({\WS}) WQA-U & +0.0\% \\ % 0
        %\textbf{(Ours)} T5-large & ({\WS}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$  & +3.2\% \\ % +3.219056816
        %\textbf{(Ours)} T5-large & ({\WS}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO}) WQA-L$_{\text{Train}}$ & +4.8\% \\ % +4.81248994
        %\textbf{(Ours)} T5-large & ({\WS}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}) WQA-L$_{\text{Train}}$ & +11.3\% \\ % +11.26669886
        %\textbf{(Ours)} T5-large & ({\WS}+{\SCO}) WQA-U $\rightarrow$ ({\WS}+{\LW}+{\SCO})  WQA-L$_{\text{Train}}$ & +10.1\% \\ % +10.07564784
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of $\text{WQA}_{\text{L}}$ for different training paradigms of GenQA models. All results are reported in relative \% changes w.r.t the AS2 baseline.
%    }
%    \label{tab:wqa_results}
%\end{center}
%\end{table*}

%\begin{table*}
%\small
%\begin{center}
 %   \resizebox{0.9\linewidth}{!}{
 %   \begin{tabular}{lcccc} 
 %       \toprule
 %       Model & Teacher$\rightarrow$WQA-L & Transfer$\rightarrow$ WQA-U & Supervised$\rightarrow$ WQA-L & Accuracy \\
 %       \toprule
 %       Electra-large & AS2 &          &              &  Baseline \\
 %       \midrule
 %       T5-base      &      & WS       &              & +2.16\% \\
 %       T5-base      &      & WS+LW    & WS+LW        & +6.6\% \\
 %       T5-base      &      & WS+LW+SC & WS+LW+SC     & +11.8\% \\
 %       \midrule
 %       T5-large     &      & WS       & WS           & +0.0\% \\
 %       T5-large     &      & WS       & WS+LW        & +3.2\% \\
 %       T5-large     &      & WS       & WS+LW+SCO    & +4.8\% \\
%        T5-large     &      & WS+SC    & WS+LW        & +11.3\% \\
%        T5-large     &      & WS+SC    & WS+LW+SC     & +10.1\% \\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of $\text{WQA}_{\text{L}}$ for different training paradigms of GenQA models. All results are reported in relative \% changes w.r.t the AS2 baseline.
%    }
%   \label{tab:wqa_results}
%\end{center}
%\end{table*}


% ========= RAW PERFORMANCE ==========
%AS2 baseline  62.13 
%LW            66.21
%LW+SCO	       69.48 
%WS            63.47

% ===== RELATIVE IMPROVEMENT =========
%AS2 baseline  +0.0
%LW            +6.6
%LW+SCO	       +11.8
%WS            +2.16

% ===== ABSOLUTE IMPROVEMENT =========
%AS2 baseline  +0.0
%LW            +4.08 
%LW+SCO	       +7.35
%WS            +1.34

% ====================================



% >>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>> RELATIVE >>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>
%{\color{red}
%\begin{table}
%\begin{center}
%    \resizebox{1\linewidth}{!}{
%    \begin{tabular}{lcccc} 
%        \toprule
%        Model & Teacher & Transfer & Supervised & Accuracy \\
%        \toprule
%        ELECTRA      &         &           &          &  AS2 baseline\\
%        \midrule
%        T5-base      & ELECTRA &  WS       &          &  +2.16\% \\
%        T5-base      & ELECTRA & WS+LW     & LW       &  +6.6\%  \\
%        T5-base      & ELECTRA & WS+LW+SCO & LW+SCO   &  \textbf{+11.8\%} \\
        %\midrule
        %T5-large     & ELECTRA & WS        & WS        &  +0.0\%  \\
        %T5-large     & ELECTRA & WS        & WS + LW   &  +3.2\%  \\
        %T5-large     & ELECTRA & WS        & WS+LW+SCO &  +4.8\%  \\
        %T5-large     & ELECTRA & WS+SCO    & WS+LW     &  +11.3\  \\
        %T5-large     & ELECTRA & WS+SCO    & WS+LW     &  +10.1\% \\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of $\text{WQA}_{\text{L}}$ for different training paradigms of GenQA models. All results are reported in relative \% changes w.r.t the AS2 baseline.}
%    \label{tab:wqa_results}
%\end{center}
%\end{table}
%}
% <<<<<<<<<<<<<<<<<<<<<<<<<<<<<<< RELATIVE <<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<<

% >>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>> ABSOLUTE >>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>
{\color{red}
\begin{table}
\begin{center}
    \resizebox{1\linewidth}{!}{
    % \begin{tabular}{lcccc} 
    %     \toprule
    %     Model & Teacher & Transfer & Supervised & Accuracy \\
    %     \toprule
    %     ELECTRA      &         &           &          &  AS2 baseline\\
    %     \midrule
    %     T5-base      & ELECTRA &  WS       &          &  +1.34\% \\
    %     T5-base      & ELECTRA & WS+LW     & LW       &  +4.08\%  \\
    %     T5-base      & ELECTRA & WS+LW+SCO & LW+SCO   &  \textbf{+7.35\%} \\
    %     %\midrule
    %     %T5-large     & ELECTRA & WS        & WS        &  +0.0\%  \\
    %     %T5-large     & ELECTRA & WS        & WS + LW   &  +3.2\%  \\
    %     %T5-large     & ELECTRA & WS        & WS+LW+SCO &  +4.8\%  \\
    %     %T5-large     & ELECTRA & WS+SCO    & WS+LW     &  +11.3\  \\
    %     %T5-large     & ELECTRA & WS+SCO    & WS+LW     &  +10.1\% \\
    % \end{tabular}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Approach}}      & \multirow{2}{*}{\textbf{Model}}                                       & & \multicolumn{2}{c}{\textbf{Unlabeled: AQAD-U}} & &  \multirow{2}{*}{\textbf{Accuracy (\%)}} \\ \cmidrule(lr){4-5}
                       &                                                               &  & \textbf{Used} & \textbf{Training Strategy}     &                                \\ \midrule
\textbf{AS2}                    & \begin{tabular}[c]{@{}c@{}}ELECTRA-Base\end{tabular} & &{\xmark}    & -                     & &        Baseline        \\
\midrule
\multirow{3}{*}{\textbf{GenQA}} & T5 - Base                                                  &  & {\cmark}    & {\WS}                & &      +1.34\%                       \\
                       & T5 - Base                                                    & & {\cmark}    & {\WS} + {\LW}       &  &    +4.08\%                       \\
                       & T5 - Base                                                    & & {\cmark}    & {\WS} + {\LW} + {\SC} &          & \textbf{+7.35\%}                          \\ \bottomrule
\end{tabular}
 }
 \vspace{-0.75em}
    \caption{\small Results on $\text{AQAD}$-${\text{L}}$ for different training paradigms of GenQA models. All results are reported in absolute \% changes w.r.t the AS2 baseline.}
    \label{tab:aqad_results}
    \vspace{-1em}
\end{center}
\end{table}
}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/bleu_eval.tex <==
%\begin{table}
%\small
%\begin{tabular}{lccc}
%\toprule
%Model &   Approach               & BLEU       & BLEU        \\
%      &                          & NLG answer & AS2 answer  \\
%\midrule
%RoBERTa-large  &                 & 34.76    & 100.0 \\
%T5-large       &  GenQA          & 46.67 & 32.690  \\
%T5-large       &  WS             & 38.47    & 65.55  \\
%T5-large       &  $WS_{LW}$      & 38.85    & 63.76  \\
%T5-large       & $WS_{LW+SCI/O}$ & 36.94    & 61.22  \\
%T5-large       & $WS_{LW+SCI/O}\rightarrow GenQA$  & 49.33    & 37.62  \\

%Gold Labels & NLG target answers                    & 100.00   & 30.97 \\
%\bottomrule
%\end{tabular}
%\caption{}
%\label{tab:bleu_targe_v0}
%\end{table}

%\begin{table}[h]
%\small
%\begin{tabular}{lccc}
%\toprule
%Transfer & Supervised  & BLEU & BLEU              \\
%              &                       & NLG answer & AS2 answer  \\
%\toprule
%             & NLG Targets            & 100.00  & 30.97 \\
%             & AS2(ASNQ)              & 34.76    & 100.0       \\
%             & GenQA                  & 46.67    & 32.690       \\
%\midrule
%    WS       &                        & 38.47    & 65.55      \\
%    LW       &                        & 38.85    & 63.76       \\
%    LW + SC  &                        & 36.94    & 61.22       \\
%\midrule
%    LW + SC & GenQA                   & 49.33    & 37.62      \\ 
%\bottomrule
%\end{tabular}
%\caption{In this table we present the results considering the BLEU score as a distance measure between our models output and the manually generated target answer. In addition we also measure the distance from the generated answers and the candidate selected by the AS2 teacher model. Note that when not specified, the we train on MS-MARCO NLG for the supervised settings, and MS-MARCO for the transfer settings.}
%\label{tab:bleu_target_v0}
%\end{table}

{\color{red}
\begin{table}
\begin{center}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcccc} 
        \toprule
        Model  & Transfer & Supervised & BLEU       & BLEU \\
           &          &            & NLG answer & AS2 answer \\
        \toprule
        %       &         &          &          & 100.00 & 30.97 \\
        RoBERTa &  -       & -          & 34.76  & 100.0 \\
        \midrule
        T5       & {\WS}       &  -       & 46.67  & 32.69 \\
        T5       & {\WS}+{\LW}    &  -       & 38.47  & 65.55  \\
        T5       & {\WS}+{\LW}+{\SC} &  -        & 38.85  & 63.76  \\
        \midrule
        T5       &   -       & \cite{hsu2021answer} & 36.94  & 61.22  \\
        T5       & {\WS}+{\LW}+{\SC} & \cite{hsu2021answer}  & 49.33  & 37.62  \\
        \bottomrule
    \end{tabular}
    }
    \caption{\small Results using BLEU as the metric for measuring performance of answer generation. We train the GenQA models on MS-MARCO NLG for the supervised setting, and MS-MARCO QA for the knowledge transfer setting.}
    \label{tab:bleu_target}
\end{center}
\end{table}
}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/datasets.tex <==
\begin{table}[ht]
\tiny
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
Dataset       &   Split    & \# of Q & QA Pairs \\
\toprule
MS-MARCO QA      & Train           & 655006   & 19543964 \\
MS-MARCO QA      & Dev             & 1000    & 29309  \\
\midrule
MS-MARCO NLG    & Train            & 153725   & 4694170 \\
MS-MARCO NLG    & Dev              & 1000     & 28353 \\
MS-MARCO NLG    & Test             & 1000     & 28529 \\
\midrule
WikiQA        & Train (clean)      &  857        & 8651  \\
WikiQA        & Dev (clean)        &  121        & 1126 \\
WikiQA        & Test               &  633        & 6165 \\
\midrule
TrecQA        & Train              & 804      & 32964 \\
TrecQA        & Dev                & 216      & 9590  \\
TrecQA        & Test               & 340      & 13416 \\
\bottomrule
\end{tabular}}
\caption{\small Datasets statistics.}
\label{tab:datasets_statistics}
\end{table}


==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/evaluation_autimaticmetrics.tex <==
\begin{table}
\tiny
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Approach/Strategy}} & \textbf{Human } && \multicolumn{3}{c}{\textbf{BERT-Score}}   && \multicolumn{2}{c}{\textbf{BLEURT}}  \\
  & \textbf{Evaluation} && \textbf{PREC} & \textbf{REC} & \textbf{F1} & & \textbf{AVG} & \textbf{STDEV} \\
\midrule
 \textbf{AS2}                                    & 0.793 && 0.876 & 0.905 & 0.890 && 0.509 & 0.225     \\
 \textbf{WS}                            & 0.799 && 0.884 & 0.903 & 0.893 && 0.520 & 0.217    \\
                                    \textbf{WS+LW}                            & 0.815 && 0.993 & 0.994 & 0.993 && 0.517 & 0.216     \\
                                    \textbf{WS+SCI}                           & 0.820 && 0.885 & 0.905 & 0.895 && 0.525 & 0.218     \\
                                \textbf{WS+SCO}                           & 0.825 && 0.884 & 0.905 & 0.894 && 0.521 & 0.221     \\
                                   \textbf{WS+LW+SC}                         & 0.837 && 0.883 & 0.901 & 0.891 && 0.512 & 0.211    \\
                                    \cite{hsu2021answer}                   & 0.826 && 0.907 & 0.911 & 0.908 && 0.555 & 0.224     \\
                                 \textbf{WS+LW+SC}+   & \multirow{2}{*}{0.853} && \multirow{2}{*}{0.994} & \multirow{2}{*}{0.996} & \multirow{2}{*}{0.995} && \multirow{2}{*}{0.559} & \multirow{2}{*}{0.221}     \\
                                  \cite{hsu2021answer} & &&&&&&\\
\midrule
\multicolumn{2}{c}{\textbf{Correlation (with Human Evaluation)}} && \multicolumn{3}{c}{\textbf{0.447}} && \multicolumn{2}{c}{\textbf{0.622}} \\
\bottomrule
\end{tabular}}
\vspace{-0.75em}
\caption{\small Results on the the testset of MS MARCO-NLG comparing human evaluation to well-known automatic evaluation metrics: BERT-Score and BLEURT. The last row shows the correlation between the human evaluation and the two automatic metrics (BERT-Score, and BLEURT), indicating that these metrics do not correlate strongly with human evaluation.}
\label{tab:automaticmetrics}
% \vspace{-1em}
\end{center}
\end{table}

%Model	Human Evaluation	BERT-SCORE	BLEURT	Correlation (BERT-Score, Human)	Correlation (BLEURT, Human)
%Pr	Re	F1	Avg	Std. Dev.
% roberta-large	& 0.793 & 0.87605 & 0.90452 & 0.88957 & 0.50947 & 0.22461 & 0.44745 & 0.62195
%t5-large-ws 	&	0.799		& 0.88422 	&	0.90323 	&	0.89315 	&	0.51951 	&	0.21706
%t5-large-lw 	&	0.815 	&	0.99253 	&	0.99408 	&	0.9933 	&	0.51732 	&	0.21617
%t5-large-sci 	&	0.82 	&	0.88527 	&	0.90535 	&	0.8947 	&	0.52469 	&	0.21765
%t5-large-sco 	&	0.825	0.88361 	&	0.90461 	&	0.89351 	&	0.52147 	&	0.22129
%t5-large-lw+sci+sco 	&	0.837 	&	0.8827 	&	0.90141 	&	0.89146 	&	0.51166 	&	0.2107
%t5-large-genqa 	&	0.826 	&	0.90696 	&	0.91071 	&	0.90848 	&	0.55517 	&	0.22446
%t5-large-lw+sci+sco+ft-genqa 	&	0.853 	&	0.99359 	&	0.99575 	&	0.99467 	&	0.55857 	&	0.22084

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/msmarco_dataset.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions \\
\toprule
train       &  153725  \\
validation  &  1000    \\
test        &  1000    \\
\bottomrule
\end{tabular}
\caption{MS-MARCO NLG dataset statistics. }
\label{tab:msmarco}
\end{table}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/msmarco_results.tex <==
%\begin{table*}
%\small
%\begin{center}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{lccc} 
%        \toprule
%        Model  & Training Paradigm & Accuracy \\
%        \toprule
%        RoBERTa-large & $\text{AS2(ASNQ)}$                                                                                                                      & 0.793 \\
        
%        T5-large      & $\text{GenQA(MS-MARCO}_{\text{NLG}}\text{)}$                                                                                            & 0.826 \\
%        T5-large      & $\text{WS(MS-MARCO, RoBERTa}_{\text{ASNQ)}}\text{)}$                                                                                    & 0.799 \\
%        T5-large      & $\text{WS}_{\text{LW}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}}\text{)}$                                                                  & 0.815 \\
%        T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}} \text{)}$                                                        & 0.837 \\
%        
%        T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}} \text{)} \rightarrow \text{GenQA(MS-MARCO}_{\text{NLG}}\text{)}$ & 0.853 \\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of MSMARCO-NLG for different training paradigms of GenQA models.
%    }
%    \label{tab:msmarco_results_v1}
%\end{center}
%\end{table*}

%\begin{table*}
%\small
%\begin{center}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{lccc} 
%        \toprule
%        Transfer  & Supervised & Accuracy \\
%        \toprule
%        -- & AS2(ASNQ)           & 0.793 \\
%        -- & GenQA(MS-MARCO NLG) & 0.826 \\
%        WS(MS-MARCO, AS2(ASNQ))  & --    & 0.799 \\
%        LW(MS-MARCO, AS2(ASNQ))  & --    & 0.815 \\
%        LW + SC (MS-MARCO, AS2(ASNQ))    & --    & 0.837 \\
%        LW + SC (MS-MARCO, AS2(ASNQ))    & GenQA(MS-MARCO NLG) & 0.853 \\
        %RoBERTa-large & $\text{AS2(ASNQ)}$                                                                                                                      & 0.793 \\
        %T5-large      & $\text{GenQA(MS-MARCO}_{\text{NLG}}\text{)}$                                                                                            & 0.826 \\
        %T5-large      & $\text{WS(MS-MARCO, RoBERTa}_{\text{ASNQ)}}\text{)}$                                                                                    & 0.799 \\
        %T5-large      & $\text{WS}_{\text{LW}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}}\text{)}$                                                                  & 0.815 \\
        %T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}} \text{)}$                                                        & 0.837 \\
        %T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{ASNQ}} \text{)} \rightarrow \text{GenQA(MS-MARCO}_{\text{NLG}}\text{)}$ & 0.853 \\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of MSMARCO-NLG for different training paradigms of GenQA models. In this setting, the teacher AS2 model is always trained on ASNQ, while the our seq2seq models are trained on MS-MARCO and MS-MARCO NLG respectively for the transfer and the supervised columns.
%    }
%    \label{tab:msmarco_results_v1}
%\end{center}
%\end{table*}

%\begin{table*}
%\small
%\begin{center}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{lcccc} 
%        \toprule
%        Model & Teacher$\rightarrow$ASNQ & Transfer$\rightarrow$ MS-MARCO & Supervised$\rightarrow$ MS-MARCO NLG & Accuracy \\
%        \toprule
%        RoBERTa & AS2 &          &   & 0.793 \\
%        \midrule
%        T5      & & WS       &       & 0.799 \\
%        T5      & & WS+LW    &       & 0.815\\
%        T5      & & WS+LW+SC &       & 0.837\\
%        \midrule
%        T5      & &          & GenQA & 0.826\\
%        T5      & & WS+LW+SC & GenQA & 0.853 \\
%        \bottomrule
%    \end{tabular}
 %   }
 %   \caption{Results on the test split of MSMARCO-NLG for different training paradigms of GenQA models. In this setting, the teacher AS2 model is always trained on ASNQ, while the our seq2seq models are trained on MS-MARCO and MS-MARCO NLG respectively for the transfer and the supervised approaches.
 %   }
%    \label{tab:msmarco_results}
%\end{center}
%\end{table*}\textbf{}

%\begin{table*}
%\begin{center}
%    \resizebox{0.6\linewidth}{!}{
%    \begin{tabular}{lcccc} 
%        \toprule
%        Model &  Transfer                       & Supervised                   & Accuracy \\
%              & ASNQ$\rightarrow$ MS-MARCO      & MS-MARCO NLG                 &          \\
%        \toprule
%        RoBERTa &                               &                              & 0.793    \\
%        \midrule
%        T5      &  AS2 $\rightarrow$ WS         &                              & 0.799    \\
%        T5      &  AS2 $\rightarrow$ WS+LW      &                              & 0.815    \\
%        T5      &  AS2 $\rightarrow$ WS+LW+SC   &                              & 0.837    \\
%        \midrule
%        T5      &                               & GenQA                        & 0.826    \\
%        T5      &  AS2 $\rightarrow$ WS+LW+SC   & GenQA                        & 0.853    \\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{}
%    \label{tab:msmarco_results_v2}
%\end{center}
%\end{table*}

% {\color{red}
% \begin{table}
% \begin{center}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccc} 
%         \toprule
%         Model & Teacher & Transfer & Supervised & Accuracy \\
%         \toprule
%         RoBERTa      &    &          &       & 0.793 \\
%         \midrule
%         T5      & RoBERTa & WS       &       & 0.799 \\
%         T5      & RoBERTa & WS+LW    &       & 0.815\\
%         T5      & RoBERTa & WS+LW+SC &       & 0.837\\
%         \midrule
%         T5      &     &              & GenQA & 0.826\\
%         T5      & RoBERTa & WS+LW+SC & GenQA & \textbf{0.853} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Results on the test split of MSMARCO-NLG for different training paradigms of GenQA models. In this setting, the teacher AS2 model is always trained on ASNQ, while the our seq2seq models are trained on MS-MARCO and MS-MARCO NLG respectively for the transfer and the supervised approaches.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table}
% }

{\color{red}
\begin{table*}
\begin{center}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Approach}}      & \multirow{2}{*}{\textbf{Model}}                                       & & \multicolumn{2}{c}{\textbf{Unlabeled: MS-MARCO QA}} & & \multicolumn{2}{c}{\textbf{Labeled: MS-MARCO NLG}}   & \multirow{2}{*}{\textbf{Accuracy (\%)}} \\ \cmidrule(lr){4-5} \cmidrule(lr){7-8}
                       &                                                               &  & \textbf{Used} & \textbf{Training Strategy \textbf{(Ours)}}     & & \textbf{Used} & \textbf{Training Strategy}   &                                \\ \midrule
\textbf{AS2}                    & \begin{tabular}[c]{@{}c@{}}RoBERTa-Large\end{tabular} & &{\xmark}    & -                     & & {\xmark}     & -                   & 79.3                           \\
\midrule
\multirow{5}{*}{\textbf{GenQA}} & T5 - Large                                                  &  & {\cmark}    & {\WS}                & & {\xmark}     & -                   & 79.9                           \\
                       & T5 - Large                                                    & & {\cmark}    & {\WS} + {\LW}         &  & {\xmark}     & -                   & 81.5                           \\
                       & T5 - Large                                                    & & {\cmark}    & {\WS} + {\SCI}        &  & {\xmark}     & -                   & 82.0                           \\
                       & T5 - Large                                                    & & {\cmark}    & {\WS} + {\SCO}        &  & {\xmark}     & -                   & 82.5                           \\
                       & T5 - Large                                                    & & {\cmark}    & {\WS} + {\LW} + {\SC} &  & {\xmark}     & -                   & 83.7                           \\
                       & T5 - Large                                                    & & {\xmark}    & -                     &  & {\cmark}     & ~\cite{hsu2021answer} & 82.6                           \\
                       & T5 - Large                                                    & & {\cmark}    & {\WS} + {\LW} + {\SC} &  &  {\cmark}     & ~\cite{hsu2021answer} & \textbf{85.3}                           \\ \bottomrule
\end{tabular}
    }
    \vspace{-0.5em}
    \caption{\small Results on the test split of MS MARCO-NLG for different training paradigms of GenQA models. The weak supervision is provided by a RoBERTa-Large AS2 model trained on ASNQ. We compare with a fully supervised GenQA baseline~\cite{hsu2021answer} trained on the train split of MS MARCO-NLG.}
    \label{tab:msmarco_results}
        \vspace{-1em}
\end{center}
\end{table*}
}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/msmarconlg_dataset.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions \\
\toprule
train       &  655006  \\
validation  &  1000    \\
\bottomrule
\end{tabular}
\caption{MS-MARCO QA dataset statistics. Notice that we used this data only to train our weak-supervised models and not for test purpose.}
\label{tab:msmarconlg}
\end{table}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/trecqa_dataset.tex <==
{\color{red}
\begin{table}[ht]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions & Answers \\
\toprule
train      & 804       & 32964 \\
validation & 216       & 9590 \\
test       & 340       & 13416 \\
\bottomrule
\end{tabular}
\caption{TrecQA dataset statistics}
\label{tab:trecqa_statistics}
\end{table}
}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/wikiqa_and_trecqa_results.tex <==
%\begin{table*}
%\small
%\begin{center}
%    \begin{tabular}{lccc} 
%        \toprule
%        Model  & Training Paradigm & Accuracy \\
%        \toprule
%        RoBERTa-large & $\text{AS2(WikiQA)}$                                                                                                            & 0.783 \\
%        T5-large      & $\text{GenQA(WikiQA)}$                                                                                                          & 0.729 \\
%        T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{WikiQA}} \text{)}$                                              & 0.787 \\
%        \bottomrule
%    \end{tabular}
%    \caption{Results on the test split of WikiQA for different training paradigms of GenQA models.
%    }
%    \label{tab:wikiqa_results_v0}
%\end{center}
%\end{table*}


%\begin{table}
%\begin{center}
 %   \begin{tabular}{lccc} 
%        \toprule
%        Transfer  & Supervised & Accuracy \\
%        \toprule
%              & AS2   & 0.783 \\
%              & GenQA & 0.729 \\
%        LW+SC &       & 0.787 \\
        %RoBERTa-large & $\text{AS2(WikiQA)}$                                                                                                            & 0.783 \\
        %T5-large      & $\text{GenQA(WikiQA)}$                                                                                                          & 0.729 \\
        %T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{WikiQA}} \text{)}$                                              & 0.787 \\
%        \bottomrule
%    \end{tabular}
%    \caption{Results on the test split of WikiQA for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models direcWSy on the target dataset, while for the WS ones we used% MS-MARCO and the AS2 model in the table as a teacher. 
%    }
%    \label{tab:wikiqa_results}
%\end{center}
%\end{table}

%\begin{table}
%\begin{center}
%   \resizebox{1\linewidth}{!}{
%   \begin{tabular}{lccc} 
%       \toprule
%        Teacher & Transfer & Supervised & Accuracy \\
%        \toprule
%        AS2   &          &            & 0.783  \\
%              &          & GenQA      & 0.729\\
%       AS2   & WS+LW+SC &            & 0.787\\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of WikiQA for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models direcWSy on the target dataset, while for the WS ones we used MS-MARCO and the AS2 model in the table as a% teacher.}
%    \label{tab:wikiqa_results}
%\end{center}
%\end{table}

% {\color{red}
% \begin{table}
% \begin{center}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccc} 
%         \toprule
%         Model & Teacher & Transfer & Supervised & Accuracy \\
%         \toprule
%         RoBERTa      &    &          &       & 0.783 \\
%         T5      & RoBERTa & WS+LW+SC &       & \textbf{0.787} \\
%         T5      &         &          & GenQA & 0.729 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Results on the test split of WikiQA for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models directly on the target dataset, while for the WS ones we used MS-MARCO and the AS2 model in the table as a teacher.}
%     \label{tab:wikiqa_results}
% \end{center}
% \end{table}
% }

%\begin{table*}
%\small
%\begin{center}
%    \begin{tabular}{lccc} 
%        \toprule
%        Model  & Training Paradigm & Accuracy \\
%        \toprule
%        RoBERTa-large & $\text{AS2(TrecQA)}$                                                                                                            & 0.859 \\
%        T5-large      & $\text{GenQA(TrecQA}_{\text{L}}\text{)}$                                                                                        & 0.807 \\
%        T5-large      & $\text{WS}_{\text{LW+SCI\&SCO}}\text{(MS-MARCO, RoBERTa}_{\text{TrecQA}} \text{)}$                                              & 0.905 \\
%        \bottomrule
%    \end{tabular}
%    \caption{Results on the test split of TrecQA for different training paradigms of GenQA models.
%    }
%    \label{tab:trecqa_results_v0}
%\end{center}
%\end{table*}


%\begin{table}
%\begin{center}
   % \begin{tabular}{lccc} 
  %      \toprule
  %      Transfer  & Supervised & Accuracy \\
  %      \toprule
  %      --    & AS2   & 0.859 \\
  %      --    & GenQA & 0.807 \\
 %       LW+SC & --    & 0.905 \\
%        \bottomrule
%    \end{tabular}
%    \caption{Results on the test split of TrecQA described in Sec.~\ref{ssec:datasets} for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models direcWSy on the target dataset, while for the WS ones we used MS-MARCO and the AS2 model in the table as a teacher.}
 %   \label{tab:trecqa_results}
%\end{center}
%\end{table}

%\begin{table}
%\begin{center}
 %   \resizebox{1\linewidth}{!}{
 %   \begin{tabular}{lccc} 
 %       \toprule
 %       Teacher & Transfer & Supervised & Accuracy \\
 %       \toprule
 %       AS2   &          &            & 0.859  \\
 %             &          & GenQA      & 0.807\\
%        AS2   & WS+LW+SC &            & 0.905\\
%        \bottomrule
%    \end{tabular}
%    }
%    \caption{Results on the test split of TrecQA described in Sec.~\ref{ssec:datasets} for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models direcWSy on the target dataset, while for the WS ones we used MS-MARCO and the AS2 model in the table as a teacher.}
%     \label{tab:trecqa_results}
%\end{center}
%\end{table}

% \begin{table}
% \begin{center}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcccc} 
%         \toprule
%         Model & Teacher & Transfer & Supervised & Accuracy \\
%         \toprule
%         RoBERTa      &    &          &       & 0.859 \\
%         T5      & RoBERTa & WS+LW+SC &       & \textbf{0.905} \\
%         T5      &         &          & GenQA & 0.807 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Results on the test split of TrecQA described in Sec.~\ref{ssec:datasets} for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models direcWSy on the target dataset, while for the WS ones we used MS-MARCO and the AS2 model in the table as a teacher.}
%      \label{tab:trecqa_results}
% \end{center}
% \end{table}

% \begin{table}
% \begin{center}
% \resizebox{\linewidth}{!}{
%     \begin{tabularx}{\columnwidth}{lXc} 
%         \toprule
%         Model && Accuracy \\
%         \toprule
%         AS2     && 0.859 \\
%         \citet{hsu2021answer}  && 0.807 \\      
%         Ours  && \textbf{0.905} \\
%         \bottomrule
%     \end{tabularx}
%     }
%     \caption{Results on the test split of TrecQA described in Sec.~\ref{ssec:datasets} for different training paradigms of GenQA models. The AS2 model is a RoBERTa-large while the other approaches use a T5-large model. We train the supervised models directly on the target dataset, while for our weakly supervised model we use a weak supervised model with {\LW}+{\SC} and we train MS-MARCO and the AS2 model in the table as a teacher.}
%      \label{tab:trecqa_results}
% \end{center}
% \end{table}



\begin{table}[t]
\begin{subtable}{\linewidth}
\centering
\resizebox{\linewidth}{!}{
   \begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Approach}}                                             & & \multicolumn{2}{c}{\textbf{Unlabeled (\small{MS-MARCO QA})}} & & \multicolumn{2}{c}{\textbf{Labeled (\small{WikiQA Train}) }}   & \multirow{2}{*}{\textbf{Accuracy (\%)}} \\ \cmidrule(lr){3-4} \cmidrule(lr){6-7}
                       &                                                               & \textbf{Used} & \textbf{Training Strategy}     & & \textbf{Used} & \textbf{Training Strategy}   &                                \\ \midrule
\textbf{AS2}                    &  &{\xmark}    & -                     & & {\cmark}     & Fine-tuning            & 78.3                           \\
\midrule
\multirow{5}{*}{\textbf{GenQA}}                                                &  & {\cmark}    & {\WS} + {\LW} + {\SC}               & & {\xmark}     & -                   & 78.7                           \\
                       
                                                                       & & {\xmark}    & -                     & & {\cmark}     & ~\cite{hsu2021answer} & 72.9                           \\
                                                                         & & {\cmark}    & {\WS} + {\LW} + {\SC} &&  {\cmark}     & ~\cite{hsu2021answer} & \textbf{79.8}                           \\ \bottomrule
\end{tabular}}
   \caption{WikiQA}\label{tab:wikiqa}
\end{subtable}

\bigskip

\begin{subtable}{\linewidth}
\centering
\resizebox{1\linewidth}{!}{
   \begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Approach}}                                       & & \multicolumn{2}{c}{\textbf{Unlabeled (\small{MS-MARCO QA})}} & & \multicolumn{2}{c}{\textbf{Labeled (\small{TREC-QA})}}   & \multirow{2}{*}{\textbf{Accuracy (\%)}} \\ \cmidrule(lr){3-4} \cmidrule(lr){6-7}
                       &                                                              & \textbf{Used} & \textbf{Training Strategy}     & & \textbf{Used} & \textbf{Training Strategy}   &                                \\ \midrule
\textbf{AS2}                    &  &{\xmark}    & -                     & & {\cmark}     & Fine-tuning            & 85.9                           \\
\midrule
\multirow{5}{*}{\textbf{GenQA}} 
&  & {\cmark} & {\WS} + {\LW} + {\SC} & & {\xmark} & - & \textbf{90.5} \\ 
&  & {\xmark} & - & & {\cmark} & ~\cite{hsu2021answer} & 80.7 \\
&  & {\cmark} & {\WS} + {\LW} + {\SC} && {\cmark} & ~\cite{hsu2021answer} & 89.8  \\ %TO CHANGE? 
\bottomrule
\end{tabular}}
   \caption{TREC-QA}\label{tab:trecqa}
\end{subtable}
\caption{\small Results on the test split of WikiQA and TREC-QA. The weak supervision is provided by RoBERTa-Large AS2 models trained respectively on WikiQA and TREC-QA. We compare with a fully supervised GenQA baseline~\cite{hsu2021answer} trained respectively on the train split of WikiQA and TREC-QA using ground truth correct answers as the target for generation. We use T5-Large for all GenQA models.} \label{tab:wiki_trec}
\vspace{-0.5em}
\end{table}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/Tables/wikiqa_dataset.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions & Answers \\
\toprule
train      &  2118       & 20360  \\
validation &  296        & 2733 \\
test       &  633        & 6165 \\
\bottomrule
\end{tabular}
\caption{WikiQA dataset statistics}
\label{tab:wikiqa_statistics}
\end{table}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/analysis.tex <==

\paragraph{Automatic Evaluation:} We consider whether automatic evaluation metrics correlate with human evaluation for our task. In Table \ref{tab:automaticmetrics}, we compare BERT-Score~\cite{Zhang*2020BERTScore:} and BLEURT~\cite{sellam-etal-2020-bleurt} with the human  evaluation of various models on MS MARCO-NLG test data. We find that despite their good performance for other NLG tasks neither metric has a particularly strong Pearson correlation with the human evaluation results for the task of answer sentence generation (GenQA): BLEURT has a correlation 0.622; BERT-Score has a correlation of 0.447. Neither automatic metric is able to correctly identify the system ranking effected by human evaluation as presented in Table~\ref{tab:msmarco_results}. Additional analysis using the BLEU score is presented in Appendix~\ref{apx:acc_vs_bleu}.

\input{Tables/evaluation_autimaticmetrics}

\paragraph{Structured Output and Accuracy:} In the {\SCO} approach we propose, we prepend a special bucket token $b_1 = \mathcal{F}(q,c_{M_1})$ corresponding to the AS2 confidence score of the target answer candidate $c_{M_1}$, so that the output target for the GenQA model {\MG} is: ``$b_1 \ c_{M_1}$''. We denote the bucket tokens for $l{=}5$ with the following set: [{\tiny{\YES},{\PROBABLY},{\MAYBE}, {\DOUBT},{\NO}}] corresponding to the confidence intervals $[0.8,1]$, $[0.6,0.8)$, $[0.4, 0,6)$, $[0.2,0.4)$ and $[0,0.2)$ for {\MA}'s score respectively. In this section, we analyze the role of the {\SCO} bucket tokens as a confidence measure for the GenQA model's output during inference. For this, we cluster the answers generated by the GenQA model (a T5-Large model trained on MS-MARCO QA using both {\LW} and {\SC}) based on the generated {\SCO} bucket token. We then manually evaluate the answers and show the accuracy for each cluster in Table~\ref{tab:sco_confidence_greedy}. Here we observe an evident difference in the correctness of the generated answers in the {\YES} cluster from those in the {\NO} cluster (78.6\% v/s 60.5\%). The accuracy of generated answers monotonically decreases with the confidence interval of the bucket token ({\YES} $\rightarrow$ {\NO}). Additional analysis of model outputs is presented in Appendix~\ref{apx:quality_eval}.

\input{Tables/apx_sco_confidence}
\input{plots/apx_bleu_generated_vs_candidates}

\paragraph{Generated Answer v/s Input Candidates:} We compare the generated answers (for each {\SCO} bucket token) with the input answer candidates to understand how the model copies from the input candidates, and if there is a correlation with the {\SCO} bucket tokens. In Fig.~\ref{fig:bleu_generated_vs_candidates}, we present the similarity between the generated answer with the top $4$ ranked input candidates using BLEU score. This analysis shows that generated answers starting with a high confidence {\SCO} bucket token (e.g., {{\YES}} or {{\PROBABLY}}) are more similar to the first candidate (higher ranked), while answers starting with lower confidence {\SCO} bucket tokens (e.g., {{\NO}}) are on average equally distant from all the input candidates.




==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/bak/bkp_experiments.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training the GenQA model, we use large scale unlabeled datasets by leveraging our proposed knowledge transfer from a trained AS2 model: one public and one industrial one. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\mypara{MS-MARCO}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which has popularly been used for several NLP tasks like passage ranking, document ranking, answer generation and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the passages into individual sentence which we use as answer candidates for the AS2 model. The questions from MS-MARCO along with these unlabeled answer candidates are used for training the GenQA model. We sub-sample 1000 questions from the test set of MS-MARCO, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire test split $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer Appendix.

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least
one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in thetrain/development/test sets of WikiQA having 2118/296/236 questions respectively.

\mypara{WQA} is a large scale internal industrial QA dataset containing non-representative de-identified user
questions from a commercial virtual assistant. For our experiments, we use two splits of WQA: WQA-U and WQA-L which correspond to large unlabeled and a small labeled split respectively. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. WQA-L contains questions with answer candidates retrieved similar to WQA-U having human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively. We use WQA-U and train split of WQA-L for training the GenQA model; and the test split of WQA-L for evaluation.  Results on WQA are presented relative to the baseline AS2 model due to
the data being internal. For complete details and data statistics, refer Appendix.


\subsection{Models and Baselines}
For the GenQA model {\MG}, we use the T5-Base and T5-Large~\cite{raffeletall2020} variants of the UnifiedQA (T5UQA) model released by ~\citet{khashabi-etal-2020-unifiedqa}. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision @ 1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 
We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
\label{ssec:Results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/bak/bkp_experiments_042022.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training our model, we use large scale unlabeled datasets -- a public dataset with $\sim$800K questions and a larger industrial dataset of $\sim$50M. When available, we finetune on labeled data sources with and without a transfer step. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\subsubsection{Unlabeled Data}
\mypara{MS-MARCO Question Answering}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which is often used for NLP tasks like passage ranking, document ranking, and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the original dataset into individual sentences using the BlingFire tokenizer\footnote{https://github.com/microsoft/BlingFire} to be used as answer candidates for the AS2 model. We use this data as unlabeled $(q,a)$ pairs for transferring knowledge from \MA to \MG. 

\mypara{WQA-U} is a large scale internal industrial QA dataset containing non-representative de-identified user questions from a commercial virtual assistant. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. 

\subsubsection{Labeled Data}

\mypara{MS-MARCO NLG} provides at least one manually generated answer for each question from a subset of MS MARCO Question Answering. The train split contains $\sim$ 150k (q,a) pairs.  We sub-sample 1k questions from the development set, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire development set of $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer to Appendix.

\mypara{WQA-L} is the labeled counterpart to the industrial dataset WQA-U defined above, where answer candidates have human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively.  Results on WQA-L are presented relative to the baseline AS2 model due to the data being internal. For complete details and data statistics, refer Appendix.

%\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark used to evaluate AS2 models. For our experiments, we use the filtering and splits proposed in \cite{trecqazeyu}, where all questions have at least one positive and one negative candidate and the test split is larger. The resulting dataset is composed by 816, 204, 340 unique questions respectively for train, development and test set.

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in train/development/test sets of WikiQA having 2118/296/236 questions respectively.

\subsection{Models and Baselines}
For {\MG} models, we use the base and large versions of T5~\cite{raffeletall2020}. We train these two models on two different splits of MS-MARCO: we used the MS-MARCO NLG trainset for the GenQA model, and the MS-MARCO QA training set for our weak supervised models. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model \cite{clark2020electra} trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average \todo{micro-average instead of majority voting, since the latter one provided unreliable performance.} number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision@1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
\label{ssec:experimental_details}

For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 

We train our models using $fp16$ precision, Adam \cite{Kingma2015AdamAM} as optimizer with a $lr=1e-04$ and a batch size of $256$. We trained each model for $25$ epochs on both the versions of MS-MARCO and for $50$ epochs on WikiQA and TrecQA. We select the best model by maximizing the average AS2 score on the development set of each dataset instead of minimizing the validation loss (see the details in Appendix \ref{apx:ckpt_selection}).

We perform experiments on three different settings:
\subsubsection{MS-MARCO \& MS-MARCO NLG}
With this experiment we train and evaluate our model on a well-known and large dataset. Specifically, this experiment is useful to properly understand the effectiveness of our week supervised methods and to compare them with the original supervised GenQA model. We train our models considering the unlabeled MS-MARCO dataset described in Sec.~\ref{ssec:datasets} and we use a AS2 teacher based on RoBERTa-large and trained on ASNQ for the knowledge transfer. It is important to notice that in this setting, during the training both the student and the teacher model have not any knowledge about the original labels of MS-MARCO. In contrast, the proposed baseline based on the original GenQA model \cite{hsu2021answer} is trained on MS-MARCO NLG which is labeled and also provides high quality manually generated answers. In addition, we propose a two stages training to understand if a second training on a supervised dataset could improve the performance of model trained using our weak supervision techniques. All the models are then evaluated by manual annotators on the same MS-MARCO NLG testset described in Sec.~\ref{ssec:datasets} and the results are reported in terms of accuracy.

\subsubsection{WikiQA \& TrecQA}
In this experiment, we measure the quality of our training approaches evaluating their performance on two AS2 benchmark datasets which are WikiQA and TrecQA. With this setting we explored the capability of the models by answering different research questions. Specifically, we compare our approaches with a strong AS2 baseline and a GenQA model directly trained on this dataset, to verify two hypothesis: first, our approaches can be easily applied and extended to different datasets, and second that a knowledge tranfer from an in-domain teacher could improve the performance of the teacher itself. In addition, we explore further the limitations of the traditional GenQA approach on a few data setting. To perform these experiment, we trained our approaches on a weak supervised setting using MS-MARCO and an AS2 teacher trained directly on TrecQA and WikiQA. In contrast, for the GenQA and the AS2 baseline models, we directly perform the training on the benchmarks. The models were respectively evaluated on the two test splits defined in Sec.~\ref{ssec:datasets}.


%\textcolor{red}{why this experiments?}
%\begin{itemize}
%    \item \textcolor{red}{in this setting we consider smaller datasets}
%    \item \textcolor{red}{our models have some knowledge about them (the as2 teacher model is trained on them)}
%    \item \textcolor{red}{these models does not provide manually generated answers}
%    \item \textcolor{red}{our model trained on more but unlabeled data}
%    \item \textcolor{red}{our model are improving the teacher?}
%\end{itemize}

%\textcolor{red}{setting?}
%\begin{itemize}
%    \item \textcolor{red}{our models are trained on msmarco but having a teacher finetuned on the two considered datasets (wikiqa and trecqa)}
%    \item \textcolor{red}{the hsuetall model is trained directly on the two datasets, and since the dataset have not manually generated answers, during the training we consider as target a positive answer randomly selected from the %original set of candidates}
%    \item \textcolor{red}{the teacher is an AS2 model based on roberta-large and trained directly on the two datasets.}
%    \item 
%\end{itemize}

\subsubsection{Industrial Setting: WQA}

%We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
In this section we present the results obtained on the three different settings defined in Sec.~\ref{ssec:experimental_details}.

\label{ssec:Results}

\subsubsection{MS-MARCO}
\label{sssec:msmarco_results}
\input{Tables/msmarco_results}

We present the results on the MS-MARCO NLG testset in Table~\ref{tab:msmarco_results} in terms of accuracy. The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points, which is the model with the lowest accuracy in this setting. Our transfer techniques improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with in weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point showing that our seq2seq QA models are robuster and have better generalization capabilities. In addition, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($\text{TL}_{\text{LW+SCI\&SCO}}$) by several accuracy points (0.837 vs 0.853).

%\begin{itemize}
%    \item \textcolor{red}{The AS2 baseline is the model with the lowest results, show that our generative models are robuster and present better generalization capabilities.}
%    \item \textcolor{red}{The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points. }
%    \item \textcolor{red}{Our transfer technique improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with an weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point.}
%    \item \textcolor{red}{Lastly, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($TL_{LW+SCI\&SCO}$) by several accuracy points (0.837 vs 0.853)}
%\end{itemize}


\subsubsection{WikiQA \& TrecQA}
\label{sssec:qa_results}
\input{Tables/wikiqa_and_trecqa_results}

The results presented in Table \ref{tab:wikiqa_results} and Table \ref{tab:trecqa_results} show that our Transfer Learning techniques have better performance than both the AS2 model and the GenQA baselines. Indeed, we verified the hypothesis that applying our transfer learning techniques can improve the original AS2 model used as a teacher. For examples, in both the datasets our TL model outperform the AS2 baseline by $0.04$ and $4.6$ accuracy points respectively for WikiQA and TrecQA. In addition, we proved that the original GenQA approach requires a bigger dataset to converge to a good solution and to effectively outperform the AS2 models (as we experienced in Sec.\ref{sssec:msmarco_results}).

%\todo{to write this section.}
%\begin{itemize}
%\item \textcolor{red}{TL techniques have better performance then the as2 model. Indeed, we verified the hypotesis that applying these transfer learning techniques can improve the original AS2 model used as a teacher.}
%\item \textcolor{red}{GenQA have poor performance, we can infer that this training setting requires more data to converge to a good solution.}
%\end{itemize}


\subsubsection{Industrial dataset}
\label{sssec:industrial_results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/bak/bkp_methodology.tex <==
Previous works on GenQA~\cite{hsu2021answer} require the use of labeled data: either human written high-quality natural answers, or human annotations on correctness/incorrectness of answer candidates; for effectively training the GenQA model.
Towards mitigating the requirement of large scale labeled data for training GenQA, which is very expensive to annotate, we propose a training paradigm for GenQA that only uses unlabeled data while being weakly-supervised by a discriminative AS2 model.

\subsection{Training GenQA using an AS2 model}
\label{ssec:training_genqa}

Given a trained AS2 model {\MA} which predicts correctness/incorrectness of an answer candidate for a question in a discriminative manner, we want to learn a GenQA model while only having access to unlabeled data $\mathcal{U}$. Specifically, the dataset $\mathcal{U}$ comprises of a set of questions along with their retrieved answer candidates, i.e, $(q,C=\{c_1,\dots,c_n\})$. Note that there are \emph{no} human annotations of correctness/incorrectness for the answer candidates in $C$ for the question $q$.

We use the trained {\MA} to produce a ranking over the candidates $C$ for each question $q \in \mathcal{U}$. For a question $q$, we denote the resulting ranking of candidates using {\MA} to be $C^{M_A}=\{c^{M_A}_{1},c^{M_A}_{2},\dots,c^{M_A}_{n}\}$ in decreasing order of prediction scores. Then we use this generated ranking $C^{M_A}$ as weak supervision for training the GenQA model {\MG}. We use the top ranked answer candidate $c^{M_A}_{1}$ for $q$ by {\MA} as a proxy for the human written/correctly annotated answer to be used as the output target for {\MG}. We model the generative QA problem where {\MG} takes as input the question $q$ and the set of $k$ top ranked answer candidates ranked by {\MA} after the top-1 as the context $\bar{c}$, i.e, $\bar{c}=\{c^{M_A}_{2},c^{M_A}_{3},\dots, c^{M_A}_{k+1}\}$; and predicts the top ranked answer candidate $c^{M_A}_{1}$ as the output. For seq2seq transformer-based text generation models like T5~\cite{raffeletall2020} and BART~\cite{lewis-etal-2020-bart}, we concatenate the question and $k$ answer candidates: ``$q$ [SEP] $c^{M_A}_{2}$ [SEP] $\dots$ [SEP] $c^{M_A}_{k+1}$''  to be provided as input to {\MG} and use the negative log probability of predicting each token of the target $c^{M_A}_{1}$ given the previous tokens as the training loss. 

The resulting GenQA model {\MG} is trained on the fully unsupervised dataset only using weak supervision from the discriminative AS2 model {\MA}. For the rest of the paper, we denote this training paradigm for GenQA by {\WS}. This approach is related to knowledge distillation (KD)~\cite{hinton2015distilling} wherein the predictions of a teacher model are used for guiding the learning of a student model. The novelty of our proposed approach from standard distillation techniques stems from the fact that the teacher (AS2) and student (GenQA) belong to different paradigms of training, the former being a discriminative classifier model while the latter being a generative model. Furthermore, standard KD techniques~\cite{hinton2015distilling,sanh2020distilbert} use a combination of supervision from the teacher (KL divergence) and supervision from the labeled data (Cross Entropy) for teaching the student, while in our case, we only use the supervision signal from the teacher without any access to labeled data.


\subsection{Weighting GenQA Loss via AS2 scores}
\label{ssec:lossweighting}

The binary cross-entropy loss used for training discriminative AS2 models typically calibrates their prediction w.r.t answer correctness~\cite{kamath-etal-2020-selective,garg-moschitti-2021-will}. This means that questions for which the top ranked answer from {\MA} has a higher prediction probability, are more likely to be correct than the top ranked answer for another question with a lower prediction probability. We exploit this in addition to the ranking order generated by {\MA} to improve the learning of the GenQA model {\MG}. Intuitively, we want the GenQA model to learn more from good quality target answers (having higher prediction scores) than inferior quality answers.

Specifically, we use the prediction score $\mathcal{M}_A(q,c^{M_A}_{1})$ (normalized in $[0,1]$) of {\MA} on the top ranked answer candidate to weight the loss term for {\MG} corresponding to that instance (question $q$). For a batch of questions $\mathcal{B}{=}\{(q_1,C_1),\dots,(q_m,C_m)\}$, the AS2-score weighted loss function can be presented as follows:

\begin{equation*}
    \mathcal{L}(\mathcal{B}){=}-\frac{1}{m} \sum_{i=0}^{m} w_i \cdot \mathcal{P}\Big(\mathcal{M}_G(q_i,\bar{c})=c^{M_A}_{1}\Big)
\end{equation*}
where $w_i=\mathcal{M}_A\big(q_i,c^{M_A}_{1}\big)$ is the prediction score of {\MA} for the top ranked answer candidate for $q_i$, and  $\mathcal{P}(\cdot)$ is the probability of prediction of the target answer by {\MG} given the input question and $k$ answer candidates as context. In practice, $\mathcal{P}$ is implemented as the log probability of prediction of each token of the target given previous tokens. For the rest of the paper, we will denote the AS2-score loss weighting for training GenQA as {\LW}.


\subsection{AS2 Score Conditioned I/O Shaping}
\label{ssec:SIOLF}

In the previous section, we proposed a method for incorporating the AS2 prediction score for weighting the training loss for GenQA. Alternately, the AS2 prediction score can be incorporated more implicitly for influencing the generation of the GenQA model {\MG}. This is done by means of manipulating the inputs and outputs when training the GenQA model based on the AS2 prediction score. For seq2seq transformer-based text generation models, this is closely related with incorporating and manipulating prompts for the input/output.

We define a bucketing function $\mathcal{F}$ that operates on the AS2 prediction score $\mathcal{M}_A(q,a)$ for a QA pair $(q,a)$ and assigns a confidence bucket $B{=}[b_1,\dots,b_l]$ over the normalized interval $[0,1]$. Here $\mathcal{F}\big(\mathcal{M}_A(q,a)\big)$ is assigned $b_i$ if $\mathcal{M}_A(q,a) \in \Big[\frac{i-1}{l},\frac{i}{l}\Big)$. For our experiments, we set the value of $l{=}5$, and assign a text token for each bucket $b_i \in B$ which correlates with the confidence of the bin in natural text as follows: [`yes',`probably',`maybe',`doubt',`no']. We incorporate  $\mathcal{F}$ for manipulating the input and output of the GenQA model as follows:

\begin{itemize}
    \item \textbf{AS2 Score Conditioned Input:} For each of the $k$ answer candidates to be provided as input $\bar{c}{=}\{c^{M_A}_{2},\dots, c^{M_A}_{k+1}\}$, we assign the natural text token corresponding to the bucket $b_i$ they fall in as per $\mathcal{F}$. We denote the resulting set of text tokens for $\bar{c}$ to be [$I_2,\dots,I_{k+1}$]. We modify the input to the GenQA model to be: ``$q$ [SEP] $I_2 \ c^{M_A}_{2}$ [SEP] $\dots$ [SEP] $I_{k+1} \ c^{M_A}_{k+1}$'', where each answer candidate is prefixed with the confidence bucket token. We denote this by {\SCI}.     
    \item \textbf{AS2 Score Conditioned Output:} For the target answer candidate $c^{M_A}_{1}$, we assign the natural text token corresponding to the bucket $b_i$ it falls in as per $\mathcal{F}$, which we denote by $I_1$. We modify the output target of the GenQA model to be: ``$I_1 \ c^{M_A}_{1}$'', where the target answer is prefixed with the confidence bucket token. We denote this by {\SCO}. 
\end{itemize}

{\SCI} and {\SCO} can be used independently as well as jointly for training the GenQA model {\MG} using {\MA}. {\SCO} is related to {\LW} presented in Sec~\ref{ssec:lossweighting}, but differs in explicitly forcing the generation of {\MG} to be influenced by the confidence score of {\MA}. Using {\SCO} for training {\MG} leads to the generated text starting with one of the confidence bin tokens. During inference, this can be used to estimate the confidence of {\MG} in predicted the generated answer. Furthermore, we can exploit this to control the prediction behavior of {\MG} by forcing the decoding to start from one of these special confidence bin tokens. We explore this empirically in Sec~\ref{sec:experiments}.

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/bak/experiments_Apr22_bak.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training our model, we use large scale unlabeled datasets -- a public dataset with $\sim$800K questions and a larger industrial dataset of $\sim$50M. When available, we finetune on labeled data sources with and without a transfer step. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\subsubsection{Unlabeled Data}
\mypara{MS-MARCO Question Answering}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which is often used for NLP tasks like passage ranking, document ranking, and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the original dataset into individual sentences using the BlingFire tokenizer\footnote{https://github.com/microsoft/BlingFire} to be used as answer candidates for the AS2 model. We use this data as unlabeled $(q,a)$ pairs for transferring knowledge from \MA to \MG. 

\mypara{WQA-U} is a large scale internal industrial QA dataset containing non-representative de-identified user questions from a commercial virtual assistant. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. 

\subsubsection{Labeled Data}

\mypara{MS-MARCO NLG} provides at least one manually generated answer for each question from a subset of MS MARCO Question Answering. The train split contains $\sim$ 150k (q,a) pairs.  We sub-sample 1k questions from the development set, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire development set of $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer to Appendix.

\mypara{WQA-L} is the labeled counterpart to the industrial dataset WQA-U defined above, where answer candidates have human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively.  Results on WQA-L are presented relative to the baseline AS2 model due to the data being internal. For complete details and data statistics, refer Appendix.

%\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark used to evaluate AS2 models. For our experiments, we use the filtering and splits proposed in \cite{trecqazeyu}, where all questions have at least one positive and one negative candidate and the test split is larger. The resulting dataset is composed by 816, 204, 340 unique questions respectively for train, development and test set.

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in train/development/test sets of WikiQA having 2118/296/236 questions respectively.

\subsection{Models and Baselines}
For {\MG} models, we use the base and large versions of T5~\cite{raffeletall2020}. We train these two models on two different splits of MS-MARCO: we used the MS-MARCO NLG trainset for the GenQA model, and the MS-MARCO QA training set for our weak supervised models. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model \cite{clark2020electra} trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average \todo{micro-average instead of majority voting, since the latter one provided unreliable performance.} number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision@1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
\label{ssec:experimental_details}

For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 

We train our models using $fp16$ precision, Adam \cite{Kingma2015AdamAM} as optimizer with a $lr=1e-04$ and a batch size of $256$. We trained each model for $25$ epochs on both the versions of MS-MARCO and for $50$ epochs on WikiQA and TrecQA. We select the best model by maximizing the average AS2 score on the development set of each dataset instead of minimizing the validation loss (see the details in Appendix \ref{apx:ckpt_selection}).

We perform experiments on three different settings:
\subsubsection{MS-MARCO \& MS-MARCO NLG}
With this experiment we train and evaluate our model on a well-known and large dataset. Specifically, this experiment is useful to properly understand the effectiveness of our week supervised methods and to compare them with the original supervised GenQA model. We train our models considering the unlabeled MS-MARCO dataset described in Sec.~\ref{ssec:datasets} and we use a AS2 teacher based on RoBERTa-large and trained on ASNQ for the knowledge transfer. It is important to notice that in this setting, during the training both the student and the teacher model have not any knowledge about the original labels of MS-MARCO. In contrast, the proposed baseline based on the original GenQA model \cite{hsu2021answer} is trained on MS-MARCO NLG which is labeled and also provides high quality manually generated answers. In addition, we propose a two stages training to understand if a second training on a supervised dataset could improve the performance of model trained using our weak supervision techniques. All the models are then evaluated by manual annotators on the same MS-MARCO NLG testset described in Sec.~\ref{ssec:datasets} and the results are reported in terms of accuracy.

\subsubsection{WikiQA \& TrecQA}
In this experiment, we measure the quality of our training approaches evaluating their performance on two AS2 benchmark datasets which are WikiQA and TrecQA. With this setting we explored the capability of the models by answering different research questions. Specifically, we compare our approaches with a strong AS2 baseline and a GenQA model directly trained on this dataset, to verify two hypothesis: first, our approaches can be easily applied and extended to different datasets, and second that a knowledge tranfer from an in-domain teacher could improve the performance of the teacher itself. In addition, we explore further the limitations of the traditional GenQA approach on a few data setting. To perform these experiment, we trained our approaches on a weak supervised setting using MS-MARCO and an AS2 teacher trained directly on TrecQA and WikiQA. In contrast, for the GenQA and the AS2 baseline models, we directly perform the training on the benchmarks. The models were respectively evaluated on the two test splits defined in Sec.~\ref{ssec:datasets}.


%\textcolor{red}{why this experiments?}
%\begin{itemize}
%    \item \textcolor{red}{in this setting we consider smaller datasets}
%    \item \textcolor{red}{our models have some knowledge about them (the as2 teacher model is trained on them)}
%    \item \textcolor{red}{these models does not provide manually generated answers}
%    \item \textcolor{red}{our model trained on more but unlabeled data}
%    \item \textcolor{red}{our model are improving the teacher?}
%\end{itemize}

%\textcolor{red}{setting?}
%\begin{itemize}
%    \item \textcolor{red}{our models are trained on msmarco but having a teacher finetuned on the two considered datasets (wikiqa and trecqa)}
%    \item \textcolor{red}{the hsuetall model is trained directly on the two datasets, and since the dataset have not manually generated answers, during the training we consider as target a positive answer randomly selected from the %original set of candidates}
%    \item \textcolor{red}{the teacher is an AS2 model based on roberta-large and trained directly on the two datasets.}
%    \item 
%\end{itemize}

\subsubsection{Industrial Setting: WQA}

%We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
In this section we present the results obtained on the three different settings defined in Sec.~\ref{ssec:experimental_details}.

\label{ssec:Results}

\subsubsection{MS-MARCO}
\label{sssec:msmarco_results}
\input{Tables/msmarco_results}

We present the results on the MS-MARCO NLG testset in Table~\ref{tab:msmarco_results} in terms of accuracy. The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points, which is the model with the lowest accuracy in this setting. Our transfer techniques improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with in weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point showing that our seq2seq QA models are robuster and have better generalization capabilities. In addition, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($\text{TL}_{\text{LW+SCI\&SCO}}$) by several accuracy points (0.837 vs 0.853).

%\begin{itemize}
%    \item \textcolor{red}{The AS2 baseline is the model with the lowest results, show that our generative models are robuster and present better generalization capabilities.}
%    \item \textcolor{red}{The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points. }
%    \item \textcolor{red}{Our transfer technique improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with an weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point.}
%    \item \textcolor{red}{Lastly, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($TL_{LW+SCI\&SCO}$) by several accuracy points (0.837 vs 0.853)}
%\end{itemize}


\subsubsection{WikiQA \& TrecQA}
\label{sssec:qa_results}
\input{Tables/wikiqa_and_trecqa_results}

The results presented in Table \ref{tab:wikiqa_results} and Table \ref{tab:trecqa_results} show that our Transfer Learning techniques have better performance than both the AS2 model and the GenQA baselines. Indeed, we verified the hypothesis that applying our transfer learning techniques can improve the original AS2 model used as a teacher. For examples, in both the datasets our TL model outperform the AS2 baseline by $0.04$ and $4.6$ accuracy points respectively for WikiQA and TrecQA. In addition, we proved that the original GenQA approach requires a bigger dataset to converge to a good solution and to effectively outperform the AS2 models (as we experienced in Sec.\ref{sssec:msmarco_results}).

%\todo{to write this section.}
%\begin{itemize}
%\item \textcolor{red}{TL techniques have better performance then the as2 model. Indeed, we verified the hypotesis that applying these transfer learning techniques can improve the original AS2 model used as a teacher.}
%\item \textcolor{red}{GenQA have poor performance, we can infer that this training setting requires more data to converge to a good solution.}
%\end{itemize}


\subsubsection{Industrial dataset}
\label{sssec:industrial_results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/bak/introduction_bak.tex <==
Answering questions by extracting answers from the web, while effective, comes with certain drawbacks. A single web sentence may not contain all information needed to answer a question, or may provide extraneous information unrelated to the information needs of the questioner. Being written for an entirely different purpose, web sentences might be unsuitable as answers due to style issues such as sentiment or formality, or may be structurally reliant on longer discourse context and thus awkward as standalone answers. 

In light of this, researchers have experimented with using text generation systems to answer questions (GenQA). Such generative systems often learn to extract answers from relevant paragraphs~\cite{lewis-etal-2020-bart} or to summarize and synthesize information from the top candidates of an answer sentence selection (AS2) system~\cite{hsu2021answer}. Initial results have shown improvements in terms of both answer accuracy and style suitability. Recent work has extended these techniques to multilingual domains with impressive results~\cite{DBLP:journals/corr/abs-2110-07150}. 

However, a problem for generative QA models is the difficulty of obtaining training data. Existing datasets offer limited coverage of all domains where GenQA can be applied~\cite{bajaj2018ms}, or are too small to use as training data~\cite{DBLP:journals/corr/abs-2110-07150}. Generally, collecting human-authored answers to questions given a context is significantly more expensive compared to annotating the correctness of web sentences as answers. Accordingly, there are more resources available of the latter type~\cite{wang2007jeopardy,yang2015wikiqa,garg2020tanda}. 
 
We propose to transfer the knowledge learned by an AS2 model to a generative QA system. Towards this, we learn an answer generation model using weak supervision provided by a trained AS2 model on a set of unlabeled data. Specifically, the AS2 model is used to generate a ranking over the answer candidates for each question. The top answer is used as the target, while the concatenation of the question and the next 4 top ranked answers is used as the input for the GenQA model. 

In addition to using the weak supervision from the ranking of answers provided by the AS2 model, we also exploit the prediction score for the top answer from the AS2 model by proposing 2 modifications of our training strategy. The first one weighs the training loss of each instance with the score of the top ranked answer from the AS2 model so as to selectively learn more from `good' quality answers. The second manipulates the inputs and outputs to the GenQA model by prefixing the answer candidates with a text token that corresponds to the confidence bin of their AS2 score. 

We perform empirical evaluation on three popular public: MS-MARCO, WikiQA, TREC-QA; and one large scale industrial QA dataset. Our results show that the GenQA model trained using our paradigm of weak supervision from an AS2 model can surprisingly outperform the latter. The answers provided by our GenQA model are often more directly related to the question being asked and stylistically more suitable as responses.

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/conclusion.tex <==
In this paper, we have presented a novel approach for transferring knowledge from a discriminative AS2 model to an answer generation model, only using unlabeled data. We use the ranking produced by the AS2 model for training a GenQA model using the top answer as the target output, and the next $k$ top ranked answers along with the question as the input. We also propose input/output shaping and loss weighting techniques during knowledge transfer to improve the performance of GenQA. Our experimental results on three public and one large industrial datasets show that GenQA models trained with knowledge transfer from  AS2 models achieve higher answering accuracy than both the AS2 teacher and supervised GenQA trained with in-domain data. We are releasing our code and trained models to support future research.

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/data.tex <==
For training and evaluating our knowledge transfer techniques ({\WS}, {\LW}, {\SC}) described above, we categorize the data that we use for each experiment into the following four sources/types:
\vspace{-.5em}
\begin{itemize}
    \item\textbf{AS2:} Labeled $(q,a)$ pairs with correctness and incorrectness annotation for training {\MA}
    \vspace{-.5em}
\item\textbf{Transfer:} Unlabeled $(q,a)$ pairs that are ranked by {\MA}, and used for knowledge transfer to {\MG}
    \vspace{-.5em}
\item\textbf{Fine-tuning:} Labeled data (human written answers / answers with correctness labels) for fine-tuning {\MG}, \emph{whenever available} 
\vspace{-.5em}
    \item\textbf{Evaluation:} Evaluation data for {\MA} and {\MG}
\end{itemize} 
\vspace{-.5em}

\noindent In Section~\ref{sec:experiments}, we vary the sources of different types of the data described above, to demonstrate the robustness and generality of our knowledge transfer method. Below, we provide details about the data sources we use, along with a summary of the underlying models. 

\vspace{-.4em}
\subsection{Unlabeled Data}
\vspace{-.2em}
\label{ssec:unlabeled_data}

\mypara{MS-MARCO QA} A popular MR dataset released by ~\cite{bajaj2018ms}. We use the training split which contains ${\sim}$800k unique user queries from the Bing search engine along with $\sim10$ passages retrieved for each question.\footnote{MS-MARCO v2.1:  \url{https://huggingface.co/datasets/ms_marco}} We split the original dataset into individual sentences using the BlingFire tokenizer\footnote{\url{https://github.com/microsoft/BlingFire}} to be used as the {\bf Transfer} data. Note that this dataset is used as unlabeled data for our experiments.

\mypara{AQAD-U} A large scale internal industrial QA dataset containing \emph{non-representative de-identified} user questions from Alexa virtual assistant. This unlabeled Alexa QA Dataset (AQAD-U) contains ${\sim}$50 million questions, and ${\sim}$400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. We use this dataset as {\bf Transfer} data for experiments in the industrial setting.

\vspace{-.5em}\subsection{Labeled Data}
\label{ssec:labeled_data}
\vspace{-.2em}

\mypara{ASNQ} A large-scale AS2 corpus~\cite{garg2020tanda} derived from Google Natural Questions (NQ) dataset~\cite{kwiatkowski-etal-2019-natural}. It consists of ${\sim}$60K questions with labeled answer sentences. We use this as {\bf AS2} training data. 

\mypara{MS-MARCO NLG} A split of MS-MARCO~\cite{bajaj2018ms} that contains manually generated answers along with retrieved passages for ${\sim}$150k user queries, which we use for {\bf Fine-tuning}. We sub-sample 1k questions from the development set, along with their answer candidates extracted from the associated passages, to be used as \textbf{Evaluation} data in our experiments. (We do not use the entire development set of $\sim$ 100k questions for evaluation due to the expensive cost of human annotations).

\mypara{TREC-QA} A popular QA benchmark~\cite{wang2007jeopardy} used to evaluate AS2 models. For our experiments, we use the filtering and splits proposed in ~\cite{trecqazeyu}, where all questions have at least one positive and one negative candidate, and the test split is larger. The resulting dataset contains 816, 204 and 340 unique questions respectively for the training, dev.~and test sets.

\mypara{WikiQA} A popular AS2 dataset~\cite{yang2015wikiqa} containing questions from Bing search logs and answer candidates from Wikipedia. We use a `clean' setting for training by retaining questions with at least one positive answer candidate in the train and validation splits. This results in training/dev./test sets of WikiQA having 2118/296/236 questions, respectively.

\mypara{AQAD-L} The labeled counterpart of the industrial dataset AQAD-U as described in Section~\ref{ssec:unlabeled_data} above, where answer candidates additionally have human annotations of correctness/incorrectness. We use AQAD-L, comprising of ${\sim}$ 5k questions, as \textbf{Evaluation} data for experiments in the industrial setting. Results on AQAD-L are presented relative to the baseline AS2 model due to the data being internal. 

For data statistics, please refer to Appendix~\ref{ref:apx_data_statistics}.

\vspace{-.5em}
\subsection{Modeling Details}
\vspace{-.2em}
We use T5~\cite{raffeletall2020} as the model for GenQA {\MG}. For the AS2 models, we use a RoBERTa-Large~\cite{liu2019roberta} or ELECTRA-Base~\cite{clark2020electra} trained using the TANDA approach~\cite{garg2020tanda}, depending on the experimental setting. For our experiments, we set the value of $k{=}5$, i.e, the number of answer candidates to be provided as input to the GenQA model. 

We train our models using $fp16$ precision, Adam \cite{Kingma2015AdamAM} as optimizer with a $lr=1e{-}4$ and a batch size of $256$. We trained each model for $25$ epochs on both the versions of MS-MARCO (QA and NLG), and for $50$ epochs on WikiQA and TrecQA. We select the best model by maximizing the average AS2 score on the development set of each dataset instead of minimizing the validation loss (see the details in Appendix \ref{apx:ckpt_selection}).

\vspace{-.5em}
\subsection{Evaluation and Metrics}
\vspace{-.2em}
We perform human evaluation of our generated answers: for each question/answer pair, we collect the annotations from five annotators (corresponding to the answer being correct/incorrect) using Amazon MTurk (see Appendix~\ref{apx:maneval} for details). We use accuracy as the primary metric for all our experiments and models. Given a set of questions, this is computed as the fraction of correct answers divided by the number of incorrect answers as judged by the annotators. Note that: (i) each QA pair receives an average score from five annotators, and (ii) for the AS2 model, the accuracy is the same as Precision@1, which is the precision of the top ranked answer candidate.

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/experiments.tex <==
We perform experiments in three data settings to evaluate different features of our method. On the MS-MARCO datasets, we show that weak supervision can augment strong models trained on in-domain data. On WikiQA and TREC, we show that weak supervision on large data improves over direct supervision on small data for this QA task. We also present an experiment on a very large industrial dataset to measure the contribution of each of our proposed techniques for using unlabeled training data at scale. 

\input{Tables/msmarco_results}

\vspace{-.5em}
\subsection{Comparison with the State of the art}
\vspace{-.2em}
These experiments aim at (i) understanding the effectiveness of our weakly supervised methods ({\WS}, {\LW} and {\SC}), and (ii) comparing them with a GenQA state-of-the-art model, which is trained using fully supervised training data. We create weakly supervised data with a RoBERTa-Large AS2 model trained on ASNQ by applying it to the MS-MARCO QA dataset. It is important to note that, in this setting, during the training, both the student and the teacher models do not have any knowledge of the original labels of MS-MARCO QA as we  consider this dataset to be unlabeled. We compare our approach against a supervised GenQA model baseline~\cite{hsu2021answer}, which is trained on MS-MARCO NLG. The MS-MARCO NLG dataset is much smaller than MS-MARCO QA but has higher quality answers as the targets since they are manually written. 
We also investigate a two-stage training strategy, by first applying our knowledge transfer approach, followed by the supervised training to understand if the two approaches are complementary or essentially capture similar information. All models are evaluated by manual annotators on the same MS-MARCO NLG test set. \vspace{-1em}

\paragraph{Results:} We present the results on the MS-MARCO NLG test set in Table~\ref{tab:msmarco_results}. The baseline zero-shot accuracy of the AS2 model on this data is 79.3 and the baseline accuracy of the fully supervised GenQA model~\cite{hsu2021answer} is 82.6. Our weak supervision ({\WS}) transfer technique, which does not use any answers written by annotators as targets, shows improvements over the AS2 baseline (0.6\%). This shows that our approach can transfer information learned by an AS2 model from ASNQ (a large labeled dataset) into a GenQA model.

Ablating each of the approaches ({\LW},{\SCI},{\SCO}) individually in addition to {\WS}, we observe consistent improvements (+1.6, +2.1 and +2.6\% respectively) over the performance of {\WS}, indicating that the AS2 scores can help in the knowledge transfer. Additionally, combining all the approaches with {\WS} significantly improves the performance, and surprisingly can even outperform the supervised GenQA baseline (by 1.1\% = 83.7{-}82.6). This shows that the knowledge transferred by our approach from ASNQ exceeds what can be learned from MS-MARCO NLG.\footnote{MS-MARCO NLG is larger than ASNQ, but the latter is a much higher quality dataset in terms of diversity and complexity of questions and answer annotations}

Finally, when we combine our weak supervised training techniques with the supervised training in a two stage pipeline, we observe very significant performance gains, e.g., 2.7\% over the supervised approach. This shows that (i) the information in MS-MARCO NLG is complementary to the knowledge transferred from ASNQ, and (ii) our approach is effective in  transferring knowledge from a discriminative ranker to a downstream GenQA model.

Due to brevity of space, we present a qualitative ablation of the generated examples in Appendix~\ref{apx:quality_eval}.


\input{Tables/wikiqa_and_trecqa_results}
\vspace{-.6em}
\subsection{Scarce Data Setting}
\vspace{-.3em}
In this experiment, we measure the quality of our weak supervision approaches, by evaluating their performance on two popular AS2 benchmark datasets: WikiQA and TREC-QA. We train the AS2 teacher model on this data and still use the unlabeled data from MS-MARCO QA for performing the knowledge transfer. This way, we test if our approach is applicable in real scenarios, where data can be scarce and no large labeled data dataset is available (such as ASNQ or MS-MARCO NLG). Additionally, we verify if our approach works for other domains and if fine-tuning GenQA on the target domain data can help knowledge transfer in that domain, even in case of data scarcity.

We compare our weakly-supervised approaches with an AS2 baseline and a GenQA model trained on the target datasets, using their ground-truth labels. We used the original test splits of the datasets. Note that for these experiments, (i) we use the best performing strategy for our transfer learning, i.e.,  {\WS} along with {\LW} and {\SC}, and (ii) the AS2 baseline is the same model that we use to transfer knowledge on the MS-MARCO QA. \vspace{-.5em}

\paragraph{Results:} From our results in Table \ref{tab:wiki_trec}, we make the following observations:\\
(i) AS2 accuracy evaluated with our human annotations is around 10\% lower than results from previous works, e.g., \cite{zhang-etal-2021-joint}. As we use the same model,\footnote{Starting from the  \url{https://huggingface.co/roberta-large} checkpoint} the difference is due to the fact that we use the `raw' test setting which  includes questions with no correct answer candidates.\\ 
(ii) Our transfer learning techniques have better performance than both the AS2 model and the supervised GenQA baselines. For WikiQA, our knowledge transfer approach, which has only seen unlabeled MS-MARCO data and no labeled training data from WikiQA, gets higher accuracy than both the AS2 baseline (+0.4\%) and a fully supervised GenQA baseline (+5.8\%), which uses the ground truth labels from the target datasets. \\ 
(iii) We observe the same trend for TREC-QA: our weakly supervised models improve over both AS2 (4.6\%) and supervised GenQA (9.8\%) baselines.\\
(iv) In contrast to our observations from Table~\ref{tab:msmarco_results}, the supervised GenQA baseline for WikiQA and TREC-QA is less accurate than the AS2 baseline. We explain this with two reasons: (a) the small size of these datasets (only few thousands training questions) might be insufficient to train a large T5 model for GenQA, and (b) the usage of extracted answers as the target for generation instead of a human-written and natural sounding answer affects the quality of answer generation.\\
(v) Finally, supervised fine-tuning applied after our transfer learning only improves performance on WikiQA. The WikiQA dataset has several questions with no correct answers (${\sim}$40\%). Fine-tuning on the supervised dataset reinforces the training of the generator on questions having actual positive labels, thereby helping to reduce noise, and improving the final accuracy on the entire test set.

\vspace{-.5em}\subsection{Industrial Setting}

In this experiment, we aim to show that our experimental findings extend to very large-scale and real-world data, i.e., \emph{non-representative de-identified} customer questions from Alexa virtual assistant. We use the 50M question AQAD-U corpus as the unlabeled QA corpus for training the GenQA model, transferring the knowledge of an AS2 teacher model (no human-authored answer is used for training fully-supervised GenQA models on this data). We compare our methods for weak supervision against the AS2 teacher model on the labeled test split: AQAD-L.
\vspace{-.5em}

\paragraph{Results:}
We present the results in Table~\ref{tab:aqad_results} relative to the AS2 baseline, due to the data being internal, which is used as the `teacher' for transferring knowledge to train the GenQA model. For these experiments we use T5-Base as the GenQA model (due to the large size of AQAD-U), and our results show that knowledge transfer from the AS2 model using the unlabeled data surprisingly improves the accuracy of the baseline by 1.34\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 teacher itself. Furthermore, using loss weighting ({\LW}) and input/output shaping ({\SC}) significantly improves our weak supervision approach. The T5-Base model trained using a combination of {\LW} and {\SC} on the unlabeled AQAD-U corpus achieves an impressive 7.35\% gain in accuracy over the baseline AS2 model (which has been trained on labeled data with annotations for answer correctness). 

\input{Tables/aqad_results}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/introduction.tex <==
In recent times, extractive QA research can be categorized into two broad directions for the task of producing the final answer for a question: (i) Answer Sentence Selection (AS2), which, given a question and a set of answer-sentence candidates, selects sentences (e.g., retrieved by a search engine) that correctly answer the question; and (ii) Machine Reading (MR), e.g., \cite{Chen-Fisch-2017}, which, given a question and a reference text, involves finding an exact text span that answers the question.
AS2 models can perform more efficiently with large text databases (as they originated from the TREC-QA track \cite{voorhees99trec}), and there seems a renewed research interest in these models for applications to personal assistants, e.g., Alexa \cite{garg2020tanda,DBLP:conf/sigir/MatsubaraVM20,garg-moschitti-2021-will}.  

Both approaches (AS2 and MR) when applied for QA over unstructured web text, while effective, may have certain drawbacks. Arbitrary web sentences may not contain all the information needed to answer a question, or may contain distracting extraneous information. Moreover, they may have a particular sentiment or style that is not suited to QA, or be too structurally reliant on longer discourse context to serve as a standalone answer. 
In light of this, researchers have been exploring text generation systems for writing `better' answers. For example, in MR, RAG~\cite{10.5555/3495724.3496517} generates an answer from a set of documents selected by dense passage retrieval models.

For AS2 systems, research has focused on learning to summarize answers from relevant paragraphs~\cite{lewis-etal-2020-bart}, or to synthesize information from the top ranked candidates of an AS2 system~\cite{hsu2021answer}. The latter approach, termed as GenQA, has shown improvements in terms of both answer accuracy and style suitability. 
A distinctive characteristic of GenQA over a generation-based approach for MR is the length of the answer: the former uses an entire sentence as the target, while the latter in practice uses a short text (primarily targeting entity names). In this work, we focus on GenQA as we are interested to generate complete answer sentences from precise information selected by AS2 models.

A challenge for training effective GenQA models is the difficulty of obtaining large-scale, high-quality training data. Producing such data for GenQA typically requires human annotators to read questions and paragraphs of relevant background information, and then author a self-contained, natural answer (typically a sentence). This fairly involved procedure highly diminishes the velocity of annotation. Existing datasets in research works either offer limited coverage of all domains, where GenQA can be applied~\cite{bajaj2018ms}, or are too small to be used as supervised training data~\cite{DBLP:journals/corr/abs-2110-07150}. Generally, collecting a human-authored answer to a question when given a context is significantly more expensive compared to annotating the correctness of an extracted web sentence as an answer for the same question. Consequently, there are a large number of annotated datasets~\cite{wang2007jeopardy,yang2015wikiqa,garg2020tanda} available for the latter type, aimed at training answer sentence selection (AS2) systems.
 
In this work, we propose a training paradigm for transferring the knowledge learned by a discriminative AS2 ranking model to train an answer generation QA system. Towards this, we learn a GenQA model using weak supervision provided by a trained AS2 model on a unlabeled data set comprising of questions and answer candidates. Specifically, for each question, the AS2 model is used to rank a set of answer candidates without having any label of correctness/incorrectness for answering the question. The top ranked answer is used as the generation target for the GenQA model, while the question along with the next $k$ top-ranked answers are used as the input for the GenQA model.

We supplement the ranking order of answer candidates with the prediction confidence scores provided by the AS2 model for each answer candidate. This is done by modifying our knowledge transfer strategy in two ways. First, we weight the loss of each training instance (question + context, comprised of $k$ answer candidates) using the AS2 model score of the top ranked answer, which is to be used as the GenQA target. This allows the GenQA model to selectively learn more from `good' quality target answers in the weakly supervised training data (AS2 models are calibrated to produce higher confidence scores for correct answers). However, this loss weighting only considers the score of the output target, and does not exploit the scores of the input candidates. To overcome this limitation, we discretize and label the AS2 scores into $l$ confidence buckets, add these bucket labels to the GenQA vocabulary, and finally prepend the corresponding label to each answer candidate in the input and/or the output. This confidence bucket label provides the GenQA model with an additional signal about the answer quality of each candidate as assigned by the AS2 model. We show that both these techniques improve the QA accuracy, and can be combined to provide additional improvements.

We empirically evaluate~\footnote{We will release code and all trained models checkpoints at \url{https://github.com/amazon-research/
wqa-genqa-knowledge-transfer}} our proposed knowledge transferring technique from AS2 to GenQA on three popular public datasets: MS-MARCO NLG~\cite{bajaj2018ms}, WikiQA~\cite{yang2015wikiqa}, TREC-QA~\cite{wang2007jeopardy}; and one large scale industrial QA dataset. Our results show that the GenQA model trained using our paradigm of weak supervision from an AS2 model can surprisingly outperform both the AS2 model that was used for knowledge transfer (teacher), as well as a GenQA model trained on fully supervised data. On small datasets such as WikiQA and TREC-QA, we show that AS2 models trained even on small amounts of labeled data can be effectively used to weakly supervise a GenQA model, which then can outperform its teacher in QA accuracy. Additionally, on MS-MARCO NLG, where fully supervised GenQA training data is available, we show that an initial round of training with our weakly supervised methods yields additional performance improvements compared to the standard supervised training of GenQA. Qualitatively, the answers generated by our model are often more directly related to the question being asked, and stylistically more natural-sounding and suitable as responses than answers from AS2 models, despite being trained only on extracted sentences from the web.


==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/methodology.tex <==
Previous works on GenQA require the use of labeled data for effectively training the GenQA model.
To reduce the need of expensive large-scale training data for GenQA, we propose a training paradigm that uses unlabeled data while being weakly-supervised by a discriminative AS2 model (as shown in Fig. \ref{fig:weak_supervision}).


\vspace{-.4em}
\subsection{Answer Sentence Selection (AS2)}
\vspace{-.2em}
AS2 is a popular task in QA, defined as follows: Given a question $q$, and a set of answer candidates $C=\{c_1,\dots,c_n\}$ (retrieved using a web-index, KB, etc), find the answer candidate $c_q \in C$ that best answers $q$. This is typically modeled as a binary classifier {\MA} over QA pairs, labeled as correct or incorrect. At inference, the scores assigned by {\MA} can be used to produce a ranking over $C$, with $c_q= \text{argmax}_{i} \ \mathcal{M}(q,c_i) $. 


\vspace{-.2em}
\subsection{Generative QA (GenQA)}
\vspace{-.2em}
Generative QA refers to using a text generation model for generating an answer for a question. More specifically, when provided with a question $q$ and context $\bar{c}$, the GenQA model {\MG} should generate a natural sounding answer $c_q=\mathcal{M}_G(q,\bar{c})$ that correctly answers $q$. 
Following \citet{hsu2021answer}, we consider a set of $k$ answer candidates as the context $\bar{c}$ to be provided to {\MG}. 

\begin{figure}[t]
\includegraphics[width=\linewidth]{images/weak_supervision.png}
\centering
\vspace{-2em}
\caption{\small Our pipeline for creating weakly supervised training examples for training GenQA models. The AS2 model assigns a confidence score to each answer candidate sentence. These scores are used to select the inputs and the target sequences for the GenQA model.}
\label{fig:weak_supervision}
\vspace{-.5em}
\end{figure}



\vspace{-.2em}
\subsection{Training GenQA using an AS2 model}
\vspace{-.2em}
\label{ssec:training_genqa}

We aim at training a GenQA model, {\MG}, using a trained AS2 model, {\MA}, which predicts correctness/incorrectness of  answer candidates for a given question. Specifically, we use an unsupervised dataset, $\mathcal{U}$, comprising of a set of questions along with their retrieved answer candidates, i.e, $(q,C=\{c_1,\dots,c_n\})$. Note that there are \emph{no} human annotations of correctness/incorrectness for the answer candidates in $C$ for the question $q$.

For each question $q \in \mathcal{U}$, we denote the ranking of answer candidates by {\MA} in decreasing order of prediction scores by $C_{M}=\{c_{M_1},c_{M_2},\dots,c_{M_n}\}$. We create weakly supervised examples for training the GenQA model by using
$\big (q$, $\bar{c}=\{c_{M_2},c_{M_3},\dots, c_{M_{k+1}}\}\big)$ as the input, and setting the generation target to be the top ranked answer candidate from {\MA}, i.e, $c_{M_1}$. For seq2seq transformer-based text generation models such as T5~\cite{raffeletall2020} and BART~\cite{lewis-etal-2020-bart}, we concatenate the question and $k$ answer candidates: ``$q$ [SEP] $c_{M_2}$ [SEP] $\dots$ [SEP] $c_{M_{k+1}}$''  to be provided as input to {\MG} and use the negative log probability of predicting each token of the target $c_{M_1}$ given the previous tokens as the training loss. 


The resulting GenQA model {\MG} is trained on the unsupervised dataset only using \emph{weak supervision} from the discriminative AS2 model {\MA}. For the rest of the paper, we denote this training paradigm for GenQA by {\WS}. This approach is related to knowledge distillation (KD)~\cite{hinton2015distilling} wherein the predictions of a teacher model are used for guiding the learning of a student model. The novelty of our proposed approach from standard distillation techniques stems from the fact that the teacher (AS2) and student (GenQA) belong to different paradigms of training, the former being a discriminative classifier model while the latter being a generative model. Furthermore, standard KD techniques~\cite{hinton2015distilling,sanh2020distilbert} use a combination of supervision from the teacher (KL divergence) and supervision from the labeled data (Cross Entropy) for teaching the student, while in our case, we only use the supervision signal from the teacher without any access to labeled data.



\vspace{-.4em}
\subsection{Weighting GenQA Loss with AS2 scores}
\vspace{-.2em}
\label{ssec:lossweighting}

The binary cross-entropy loss used for training discriminative AS2 models typically calibrates their prediction w.r.t answer correctness~\cite{kamath-etal-2020-selective,garg-moschitti-2021-will}. This means that the top ranked answer to a question from {\MA} that receives a high prediction probability is more likely to be correct than the answer to another question that receives a lower prediction probability. We exploit this in addition to the ranking order generated by {\MA} to improve the learning of the GenQA model {\MG}. Intuitively, we want the GenQA model to learn more from `good' quality target answers (having higher prediction scores) than from lower quality answers.

To this end, we propose to modify our {\WS} cross-entropy loss by incorporating the AS2 scores provided by the AS2 model {\MA} when performing the knowledge transfer. Specifically, we use the prediction score $\mathcal{M}(q,c_{M_1})$ (normalized in $[0,1]$) of {\MA} on the top ranked answer candidate $c_{M_1}$ to weight the loss term for {\MG} corresponding to that instance (question $q$). Formally, the loss for each last generated word, $y_r$ of the generated output $y$ is:
\vspace{-1.5em}\\
\begin{equation}
\label{eq:lw}
\hspace{-.2em}
    \mathcal{L}_{\mathcal{M}_G}(q, c_{M_1}) = \frac{1}{Z}\mathcal{M}(q,c_{M_1}) \times \mathcal{L}_{G}(y_r,c_{M_1}), \hspace{-.5em}
\vspace{-.5em}
\end{equation}
%
%-\log \mathcal{P}(c_{M_1}|q,c_{M_2} \ldots c_{M_k}),
where $Z$ is the normalizing constant for AS2 scores computed on the training dataset, $\mathcal{L}_{G}$ is the standard loss for generating $y_r$, and $c_{M_1}$ is assumed to be the gold standard output.
$\mathcal{L}_{G}$ is defined as:
\vspace{-1.5em}\\
\begin{displaymath}
    \mathcal{L}_{G}(y_r, c_{M_{1}})=-\sum_{v\in V}log\frac{e^{y_r(v)}}{\sum_{h \in V} e^{y_r(h)}}c_{M_{1}}(r,v),
\vspace{-.5em}
\end{displaymath}
where $V$ is the vocabulary, $y_r(v)$ is the score of generating the word $v$ at position $r$, and $c_{M_{1}}(r,v)$ is 1 if the $r^{th}$ word of $c_{M_{1}}$ is $v$, otherwise it is -1.

We refer to the model trained with Eq.~\ref{eq:lw} as {\LW}.

\vspace{-.4em}
\subsection{AS2 Score Conditioned I/O Shaping}
\vspace{-.2em}
\label{ssec:SIOLF}

In the previous section, we described how to use $\mathcal{M}(q,c_{M_1})$ -- the AS2 prediction score of $c_{M_1}$ -- to weight the training loss for question $q$, since this candidate is used as the target for $q$ in {\MG}. However {\LW} ignores the AS2 scores for the other answer candidates $c_{M_2}\ldots c_{M_k+1}$, and does not explicitly provide this AS2 score as context to the GenQA model. To overcome this, we propose a method for labeling each candidate in the input of {\MG} with a representation of its AS2 score. This method can also be applied to the model output, which results in an improved performance (as shown in Section~\ref{sec:experiments}). 


We define a bucketing function $\mathcal{F}$ over the normalized interval $[0,1]$ that operates on the AS2 prediction score $\mathcal{M}(q,a)$. For a QA pair $(q,a)$, $\mathcal{F}(q,a)$ assigns a confidence bucket label $b_i \in [b_1,\dots,b_l]$ based on $\mathcal{M}(q,a)$. Here $\mathcal{F}(q,a)$ is assigned $b_i$ if $\mathcal{M}(q,a)$ is in the interval $\Big[\frac{i-1}{l},\frac{i}{l}\Big)$. For our experiments, we set the value of $l{=}5$. We add the bucket labels $b_i$ as special tokens to the vocabulary of \MG.\footnote{We experimented with using existing tokens from the vocabulary as bucket labels (e.g. ``Probably'',``Maybe'') in hopes of reusing model knowledge about the semantics of these words, but obtained worse empirical results.}

We use $\mathcal{F}$ to modify the input and output of the GenQA model as follows:
\vspace{-.5em}
\begin{itemize}
    \item \textbf{AS2 Score Conditioned Input ({\SCI}):} We prepend the bucket label $b_j = \mathcal{F}(q,c_{M_j})$ to each of the $j \in \{2,{\dots},{k{+}1}\}$ answer candidates to be provided as input to {\MG}, so that the new input is formatted as: ``$q$ [SEP] $b_2 \ c_{M_2}$ [SEP] $\dots$ [SEP] $b_{k+1} \ c_{M_{k+1}}$''.
    \vspace{-.5em}
    \item \textbf{AS2 Score Conditioned Output ({\SCO}):} We prepend the bucket label $b_1 = \mathcal{F}(q,c_{M_1})$ to the target answer candidate $c_{M_1}$, so that the output target of {\MG} is: ``$b_1 \ c_{M_1}$''. 
\end{itemize}
\vspace{-.5em}
\noindent {\SCI} and {\SCO} can be used independently as well as jointly for training the GenQA model {\MG} using {\MA}. For simplicity, we will use the acronym {\SC} when these two techniques are used together. 

We propose {\SCI} to make the knowledge transfer more effective. Intuitively, labeling each input candidate with a special token correlated with its AS2 score helps the GenQA model: during training the model can focus more on the answer candidates associated with higher quality (more correct answers), thereby improving the model performance.

While {\SCO} is related to {\LW} presented in Sec~\ref{ssec:lossweighting}, it differs in the fact that the former allows the model to ``know'' the score of the target when designing internal representations of the text in its input and output. We hypothesize that this knowledge allows the model to organize its internal representations differently in the presence of bad targets, rather than just be less influenced by them as in {\LW}. Another advantage of {\SCO} is that during inference time, we can use the generated bucket label token as a confidence score for the GenQA model's answer. Calibrating confidence scores for text generation models, e.g., using sequence likelihood, etc. is challenging, especially when decoding is constrained as in real world applications. Finally, we can force decoding to start from any one of the {\SCO} bucket tokens in order to exploit its influence on the model's output. We empirically explore this in Appendix~\ref{apx:quality_eval}.


==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/plots/apx_bleu_generated_vs_candidates.tex <==
\begin{figure}
  \centering
  \begin{tikzpicture}[scale=0.8,font=\small]
    \begin{axis}[
      width=0.95\linewidth,
      ybar,
      bar width=5pt,
      xlabel={Input candidates},
      ylabel={BLEU},
      ymin=0,
      xtick=data,
      axis x line=bottom,
      axis y line=left,
      enlarge x limits=0.15,
      symbolic x coords={c1,c2,c3,c4,all},
      legend columns=-1,
      legend style={at={(0.5,1.16)},anchor=north,legend cell align=left, nodes={scale=0.5, transform shape,draw=none}}
    ]
      \addplot[fill=green] coordinates {
            (c1,24.84)
            (c2,18.62)
            (c3,17.76)
            (c4,17.26)
            %(all,50.62)
        };
        \addplot[fill=yellow] coordinates {
            (c1,25.50)
            (c2,19.32)
            (c3,18.07)
            (c4,18.95)
            %(all,52.70)
        };
        \addplot[fill=orange] coordinates {
            (c1,25.93)
            (c2,20.84)
            (c3,19.84)
            (c4,18.13)
            %(all,53.76)
        };
        \addplot[fill=magenta] coordinates {
            (c1,25.24)
            (c2,22.03)
            (c3,21.84)
            (c4,17.47)
            %(all,48.93)
        };
        \addplot[fill=red] coordinates {
            (c1,21.71)
            (c2,21.90)
            (c3,22.40)
            (c4,22.74)
            %(all,51.50)
        };
    \legend{\YES,\PROBABLY,\MAYBE,\DOUBT,\NO}
    \end{axis}
    \end{tikzpicture}
    \vspace{-1em}
    \caption{\small Correlation between the generated answer (with different starting {\SCO} bucket tokens) with each input candidate. We observe that generated answers starting with high confidence bucket tokens (e.g., {{\YES}} and {{\PROBABLY}}) tend to copy more from the top ranked answer candidate, than the generated answers starting with lower confidence bucket tokens (e.g., {{\NO}}).}
    \label{fig:bleu_generated_vs_candidates}
\end{figure}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/plots/apx_loss_vs_rrscore.tex <==
\begin{figure}[ht!]
    \begin{center}
        \begin{tikzpicture}
        \begin{axis}[width=0.9\linewidth, xlabel=Steps, ylabel=loss (validation)]
            \addplot table [x=steps, y=devloss, col sep=comma] {csv/devloss_lwsilfsolfv3.csv};
            \addplot +[mark=none,style=dashed] coordinates {(22500, 1.22) (22500, 1.28)};
        \end{axis}
        \label{plt:devloss_ckpt}
        \end{tikzpicture}
        \begin{tikzpicture}
        \begin{axis}[width=0.9\linewidth, xlabel=Steps, ylabel=$AVG(AS2_{Score})$]
            \addplot table [x=steps, y=rrmean, col sep=comma] {csv/rr_lwsilfsolfv3.csv};
            \addplot +[mark=none,style=dashed] coordinates {(60000, 0.78) (60000, 1)};
        \end{axis}
        \label{plt:rr_ckpt}
        \end{tikzpicture}
    \caption{\small These plots show the differences between using the dev. loss and the average AS2 model score as the measure for model checkpoint selection. Notice that the vertical dashed red line is used to identify the best checkpoint (which is the one with the lowest loss in the first plot, and the one with the highest average AS2 score in the second).}
    \label{plt:checkpointselection}
    \end{center}
\end{figure}

==> Knowledge Transfer from Answer Reranking to Answer Generation (1)/related_work.tex <==
Our work builds upon recent research in AS2, answer generation for QA, and transfer learning. 

\paragraph{Answer Sentence Selection} Early approaches for AS2  use CNNs~\cite{Severyn2015LearningTR} or alignment networks~\cite{Shen2017InterWeightedAN,Tran2018TheCA,Tay2018MultiCastAN} to learn and score question and answer representations. Compare-and-aggregate architectures have also been extensively studied~\cite{Wang2017ACM,Bian2017ACM,Yoon2019ACM} for AS2. ~\citet{Madabushi2018IntegratingQC} exploited fine-grained question classification to further improve answer selection. ~\citet{garg2020tanda} achieved state-of-the-art results by fine-tuning transformer-based models on a large-scale QA dataset first, and then adapting to smaller AS2 datasets.~\citet{Matsubara2020RerankingFE} combine multiple heterogeneous systems for AS2 to improve a QA pipeline, similar in spirit to GenQA. Several follow-up works have further improved the performance of AS2 using transformer models, using multiple answer candidates~\cite{zhang-etal-2021-joint} and document-aware pre-training strategies~\cite{di-liello-etal-2022-paragraph,diliello2021pretraininingtransformersas2}.

% \todo{Are we sure there is nothing else the relwork is small. I differentiate MR from GenQA }  
\paragraph{Answer Generation for QA} Answer generation for MR has been studied by ~\citet{Izacard2021LeveragingPR,10.5555/3495724.3496517}, while ~\citet{Iida2019ExploitingBK,Goodwin2020TowardsZS,Deng2020JointLO} have studied question-based summarization (QS). ~\citet{DBLP:journals/corr/abs-2112-08688} incorporate the evidentiality of retrieved passages for training a generator, evaluated for the QA task of open-domain MR span-extraction. ~\citet{DBLP:journals/corr/abs-2110-06393} obtain extractive answer spans from a generative model by leveraging the decoder cross-attention patterns. ~\citet{fajcik-etal-2021-r2-d2} combine a generative reader with an extractive reader to aggregate evidence from multiple passages for open-domain span-extraction.

All the previously described approaches focus on identifying short answer spans for answering questions. Research on generating complete sentences as answers (similar to answer sentences produced by extractive AS2 systems) is rarer, but includes~\citet{hsu2021answer}, that propose a QA pipeline for GenQA (refer Fig~\ref{fig:genqa}). This pipeline starts with an AS2 model that selects `good' answer candidates that are then used for generating the answer. ~\citeauthor{hsu2021answer} learn to generate natural responses to questions using the top ranked candidates from the AS2 model as input context to the GenQA model. GenQA has also been explored for multilingual QA ~\cite{DBLP:journals/corr/abs-2110-07150} by extending the answer generation approach to a multilingual setting, where the answer candidates (that are used as input to the GenQA model) can be from a mix of different languages. 

In all  these works, a major challenge is finding training data for effectively training GenQA models, which requires annotator-authored natural responses. In this work, we alleviate this problem by showing that it is possible to use AS2 ranked candidates to create the input context and output target for training GenQA, achieving state-of-the-art results.



\begin{figure}[t]
\includegraphics[width=\linewidth]{images/genqa_model.pdf}
\centering
\vspace{-2em}
\caption{\small A GenQA model \cite{hsu2021answer} is a seq2seq model that takes in input a question and $k$ answer candidates, and generates an answer.}
\label{fig:genqa}
\vspace{-.2em}
\end{figure}

\vspace{-.5em}
\paragraph{Transfer Learning} Transfer learning is well studied in NLP, including pre-training~\cite{devlinetal2019,liu2019roberta}, multi-task learning~\cite{luong2015multi}, cross-lingual transfer~\cite{Schuster2019CrosslingualTL} and domain adaptation~\cite{Gururangan2020DontSP}. Our work is squarely located in this space: our underlying language models are based on pre-training for text generation~\cite{radfordetall2019gpt2,raffeletall2020}; our main contribution is to show that knowledge can be transferred sequentially from a ranking (discriminative) task to a generation task. Recently \citet{wang2021gpl} propose a new domain adaptation method leveraging large unlabeled datasets and a query generator model. \citeauthor{Izacard2021LeveragingPR} used retrieved text passages containing evidences to train a generative model for open domain QA.

==> Tables/apx_forcetokens_res.tex <==
\begin{table}[t]
\small
\begin{center}
    \begin{tabular}{lc} 
        \toprule
        Forced Starting Token & Accuracy \\
        \toprule
        \YES      &  0.767 \\
        \PROBABLY &  0.787 \\
        \MAYBE    &  0.749 \\
        \DOUBT    &  0.730 \\
        \NO       &  0.766 \\
       \bottomrule
    \end{tabular}
    \caption{Differences in accuracy measured on the WikiQA testset forcing different starting tokens. In this setting we considered a T5-large model trained using the {\LW}+{\SC} paradigm on MS-MARCO.}
    \label{tab:force_answers_res}
\end{center}
\end{table}


==> Tables/msmarco_dataset.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions \\
\toprule
train       &  153725  \\
validation  &  1000    \\
test        &  1000    \\
\bottomrule
\end{tabular}
\caption{MS-MARCO NLG dataset statistics. }
\label{tab:msmarco}
\end{table}

==> Tables/msmarconlg_dataset.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions \\
\toprule
train       &  655006  \\
validation  &  1000    \\
\bottomrule
\end{tabular}
\caption{MS-MARCO QA dataset statistics. Notice that we used this data only to train our weak-supervised models and not for test purpose.}
\label{tab:msmarconlg}
\end{table}

==> Tables/trecqa_dataset.tex <==
{\color{red}
\begin{table}[ht]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions & Answers \\
\toprule
train      & 804       & 32964 \\
validation & 216       & 9590 \\
test       & 340       & 13416 \\
\bottomrule
\end{tabular}
\caption{TrecQA dataset statistics}
\label{tab:trecqa_statistics}
\end{table}
}

==> Tables/wikiqa_dataset.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{lccc}
\toprule
Split      & Questions & Answers \\
\toprule
train      &  2118       & 20360  \\
validation &  296        & 2733 \\
test       &  633        & 6165 \\
\bottomrule
\end{tabular}
\caption{WikiQA dataset statistics}
\label{tab:wikiqa_statistics}
\end{table}

==> bak/bkp_experiments.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training the GenQA model, we use large scale unlabeled datasets by leveraging our proposed knowledge transfer from a trained AS2 model: one public and one industrial one. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\mypara{MS-MARCO}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which has popularly been used for several NLP tasks like passage ranking, document ranking, answer generation and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the passages into individual sentence which we use as answer candidates for the AS2 model. The questions from MS-MARCO along with these unlabeled answer candidates are used for training the GenQA model. We sub-sample 1000 questions from the test set of MS-MARCO, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire test split $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer Appendix.

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least
one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in thetrain/development/test sets of WikiQA having 2118/296/236 questions respectively.

\mypara{WQA} is a large scale internal industrial QA dataset containing non-representative de-identified user
questions from a commercial virtual assistant. For our experiments, we use two splits of WQA: WQA-U and WQA-L which correspond to large unlabeled and a small labeled split respectively. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. WQA-L contains questions with answer candidates retrieved similar to WQA-U having human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively. We use WQA-U and train split of WQA-L for training the GenQA model; and the test split of WQA-L for evaluation.  Results on WQA are presented relative to the baseline AS2 model due to
the data being internal. For complete details and data statistics, refer Appendix.


\subsection{Models and Baselines}
For the GenQA model {\MG}, we use the T5-Base and T5-Large~\cite{raffeletall2020} variants of the UnifiedQA (T5UQA) model released by ~\citet{khashabi-etal-2020-unifiedqa}. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision @ 1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 
We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
\label{ssec:Results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> bak/bkp_experiments_042022.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training our model, we use large scale unlabeled datasets -- a public dataset with $\sim$800K questions and a larger industrial dataset of $\sim$50M. When available, we finetune on labeled data sources with and without a transfer step. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\subsubsection{Unlabeled Data}
\mypara{MS-MARCO Question Answering}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which is often used for NLP tasks like passage ranking, document ranking, and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the original dataset into individual sentences using the BlingFire tokenizer\footnote{https://github.com/microsoft/BlingFire} to be used as answer candidates for the AS2 model. We use this data as unlabeled $(q,a)$ pairs for transferring knowledge from \MA to \MG. 

\mypara{WQA-U} is a large scale internal industrial QA dataset containing non-representative de-identified user questions from a commercial virtual assistant. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. 

\subsubsection{Labeled Data}

\mypara{MS-MARCO NLG} provides at least one manually generated answer for each question from a subset of MS MARCO Question Answering. The train split contains $\sim$ 150k (q,a) pairs.  We sub-sample 1k questions from the development set, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire development set of $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer to Appendix.

\mypara{WQA-L} is the labeled counterpart to the industrial dataset WQA-U defined above, where answer candidates have human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively.  Results on WQA-L are presented relative to the baseline AS2 model due to the data being internal. For complete details and data statistics, refer Appendix.

%\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark used to evaluate AS2 models. For our experiments, we use the filtering and splits proposed in \cite{trecqazeyu}, where all questions have at least one positive and one negative candidate and the test split is larger. The resulting dataset is composed by 816, 204, 340 unique questions respectively for train, development and test set.

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in train/development/test sets of WikiQA having 2118/296/236 questions respectively.

\subsection{Models and Baselines}
For {\MG} models, we use the base and large versions of T5~\cite{raffeletall2020}. We train these two models on two different splits of MS-MARCO: we used the MS-MARCO NLG trainset for the GenQA model, and the MS-MARCO QA training set for our weak supervised models. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model \cite{clark2020electra} trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average \todo{micro-average instead of majority voting, since the latter one provided unreliable performance.} number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision@1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
\label{ssec:experimental_details}

For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 

We train our models using $fp16$ precision, Adam \cite{Kingma2015AdamAM} as optimizer with a $lr=1e-04$ and a batch size of $256$. We trained each model for $25$ epochs on both the versions of MS-MARCO and for $50$ epochs on WikiQA and TrecQA. We select the best model by maximizing the average AS2 score on the development set of each dataset instead of minimizing the validation loss (see the details in Appendix \ref{apx:ckpt_selection}).

We perform experiments on three different settings:
\subsubsection{MS-MARCO \& MS-MARCO NLG}
With this experiment we train and evaluate our model on a well-known and large dataset. Specifically, this experiment is useful to properly understand the effectiveness of our week supervised methods and to compare them with the original supervised GenQA model. We train our models considering the unlabeled MS-MARCO dataset described in Sec.~\ref{ssec:datasets} and we use a AS2 teacher based on RoBERTa-large and trained on ASNQ for the knowledge transfer. It is important to notice that in this setting, during the training both the student and the teacher model have not any knowledge about the original labels of MS-MARCO. In contrast, the proposed baseline based on the original GenQA model \cite{hsu2021answer} is trained on MS-MARCO NLG which is labeled and also provides high quality manually generated answers. In addition, we propose a two stages training to understand if a second training on a supervised dataset could improve the performance of model trained using our weak supervision techniques. All the models are then evaluated by manual annotators on the same MS-MARCO NLG testset described in Sec.~\ref{ssec:datasets} and the results are reported in terms of accuracy.

\subsubsection{WikiQA \& TrecQA}
In this experiment, we measure the quality of our training approaches evaluating their performance on two AS2 benchmark datasets which are WikiQA and TrecQA. With this setting we explored the capability of the models by answering different research questions. Specifically, we compare our approaches with a strong AS2 baseline and a GenQA model directly trained on this dataset, to verify two hypothesis: first, our approaches can be easily applied and extended to different datasets, and second that a knowledge tranfer from an in-domain teacher could improve the performance of the teacher itself. In addition, we explore further the limitations of the traditional GenQA approach on a few data setting. To perform these experiment, we trained our approaches on a weak supervised setting using MS-MARCO and an AS2 teacher trained directly on TrecQA and WikiQA. In contrast, for the GenQA and the AS2 baseline models, we directly perform the training on the benchmarks. The models were respectively evaluated on the two test splits defined in Sec.~\ref{ssec:datasets}.


%\textcolor{red}{why this experiments?}
%\begin{itemize}
%    \item \textcolor{red}{in this setting we consider smaller datasets}
%    \item \textcolor{red}{our models have some knowledge about them (the as2 teacher model is trained on them)}
%    \item \textcolor{red}{these models does not provide manually generated answers}
%    \item \textcolor{red}{our model trained on more but unlabeled data}
%    \item \textcolor{red}{our model are improving the teacher?}
%\end{itemize}

%\textcolor{red}{setting?}
%\begin{itemize}
%    \item \textcolor{red}{our models are trained on msmarco but having a teacher finetuned on the two considered datasets (wikiqa and trecqa)}
%    \item \textcolor{red}{the hsuetall model is trained directly on the two datasets, and since the dataset have not manually generated answers, during the training we consider as target a positive answer randomly selected from the %original set of candidates}
%    \item \textcolor{red}{the teacher is an AS2 model based on roberta-large and trained directly on the two datasets.}
%    \item 
%\end{itemize}

\subsubsection{Industrial Setting: WQA}

%We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
In this section we present the results obtained on the three different settings defined in Sec.~\ref{ssec:experimental_details}.

\label{ssec:Results}

\subsubsection{MS-MARCO}
\label{sssec:msmarco_results}
\input{Tables/msmarco_results}

We present the results on the MS-MARCO NLG testset in Table~\ref{tab:msmarco_results} in terms of accuracy. The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points, which is the model with the lowest accuracy in this setting. Our transfer techniques improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with in weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point showing that our seq2seq QA models are robuster and have better generalization capabilities. In addition, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($\text{TL}_{\text{LW+SCI\&SCO}}$) by several accuracy points (0.837 vs 0.853).

%\begin{itemize}
%    \item \textcolor{red}{The AS2 baseline is the model with the lowest results, show that our generative models are robuster and present better generalization capabilities.}
%    \item \textcolor{red}{The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points. }
%    \item \textcolor{red}{Our transfer technique improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with an weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point.}
%    \item \textcolor{red}{Lastly, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($TL_{LW+SCI\&SCO}$) by several accuracy points (0.837 vs 0.853)}
%\end{itemize}


\subsubsection{WikiQA \& TrecQA}
\label{sssec:qa_results}
\input{Tables/wikiqa_and_trecqa_results}

The results presented in Table \ref{tab:wikiqa_results} and Table \ref{tab:trecqa_results} show that our Transfer Learning techniques have better performance than both the AS2 model and the GenQA baselines. Indeed, we verified the hypothesis that applying our transfer learning techniques can improve the original AS2 model used as a teacher. For examples, in both the datasets our TL model outperform the AS2 baseline by $0.04$ and $4.6$ accuracy points respectively for WikiQA and TrecQA. In addition, we proved that the original GenQA approach requires a bigger dataset to converge to a good solution and to effectively outperform the AS2 models (as we experienced in Sec.\ref{sssec:msmarco_results}).

%\todo{to write this section.}
%\begin{itemize}
%\item \textcolor{red}{TL techniques have better performance then the as2 model. Indeed, we verified the hypotesis that applying these transfer learning techniques can improve the original AS2 model used as a teacher.}
%\item \textcolor{red}{GenQA have poor performance, we can infer that this training setting requires more data to converge to a good solution.}
%\end{itemize}


\subsubsection{Industrial dataset}
\label{sssec:industrial_results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> bak/bkp_methodology.tex <==
Previous works on GenQA~\cite{hsu2021answer} require the use of labeled data: either human written high-quality natural answers, or human annotations on correctness/incorrectness of answer candidates; for effectively training the GenQA model.
Towards mitigating the requirement of large scale labeled data for training GenQA, which is very expensive to annotate, we propose a training paradigm for GenQA that only uses unlabeled data while being weakly-supervised by a discriminative AS2 model.

\subsection{Training GenQA using an AS2 model}
\label{ssec:training_genqa}

Given a trained AS2 model {\MA} which predicts correctness/incorrectness of an answer candidate for a question in a discriminative manner, we want to learn a GenQA model while only having access to unlabeled data $\mathcal{U}$. Specifically, the dataset $\mathcal{U}$ comprises of a set of questions along with their retrieved answer candidates, i.e, $(q,C=\{c_1,\dots,c_n\})$. Note that there are \emph{no} human annotations of correctness/incorrectness for the answer candidates in $C$ for the question $q$.

We use the trained {\MA} to produce a ranking over the candidates $C$ for each question $q \in \mathcal{U}$. For a question $q$, we denote the resulting ranking of candidates using {\MA} to be $C^{M_A}=\{c^{M_A}_{1},c^{M_A}_{2},\dots,c^{M_A}_{n}\}$ in decreasing order of prediction scores. Then we use this generated ranking $C^{M_A}$ as weak supervision for training the GenQA model {\MG}. We use the top ranked answer candidate $c^{M_A}_{1}$ for $q$ by {\MA} as a proxy for the human written/correctly annotated answer to be used as the output target for {\MG}. We model the generative QA problem where {\MG} takes as input the question $q$ and the set of $k$ top ranked answer candidates ranked by {\MA} after the top-1 as the context $\bar{c}$, i.e, $\bar{c}=\{c^{M_A}_{2},c^{M_A}_{3},\dots, c^{M_A}_{k+1}\}$; and predicts the top ranked answer candidate $c^{M_A}_{1}$ as the output. For seq2seq transformer-based text generation models like T5~\cite{raffeletall2020} and BART~\cite{lewis-etal-2020-bart}, we concatenate the question and $k$ answer candidates: ``$q$ [SEP] $c^{M_A}_{2}$ [SEP] $\dots$ [SEP] $c^{M_A}_{k+1}$''  to be provided as input to {\MG} and use the negative log probability of predicting each token of the target $c^{M_A}_{1}$ given the previous tokens as the training loss. 

The resulting GenQA model {\MG} is trained on the fully unsupervised dataset only using weak supervision from the discriminative AS2 model {\MA}. For the rest of the paper, we denote this training paradigm for GenQA by {\WS}. This approach is related to knowledge distillation (KD)~\cite{hinton2015distilling} wherein the predictions of a teacher model are used for guiding the learning of a student model. The novelty of our proposed approach from standard distillation techniques stems from the fact that the teacher (AS2) and student (GenQA) belong to different paradigms of training, the former being a discriminative classifier model while the latter being a generative model. Furthermore, standard KD techniques~\cite{hinton2015distilling,sanh2020distilbert} use a combination of supervision from the teacher (KL divergence) and supervision from the labeled data (Cross Entropy) for teaching the student, while in our case, we only use the supervision signal from the teacher without any access to labeled data.


\subsection{Weighting GenQA Loss via AS2 scores}
\label{ssec:lossweighting}

The binary cross-entropy loss used for training discriminative AS2 models typically calibrates their prediction w.r.t answer correctness~\cite{kamath-etal-2020-selective,garg-moschitti-2021-will}. This means that questions for which the top ranked answer from {\MA} has a higher prediction probability, are more likely to be correct than the top ranked answer for another question with a lower prediction probability. We exploit this in addition to the ranking order generated by {\MA} to improve the learning of the GenQA model {\MG}. Intuitively, we want the GenQA model to learn more from good quality target answers (having higher prediction scores) than inferior quality answers.

Specifically, we use the prediction score $\mathcal{M}_A(q,c^{M_A}_{1})$ (normalized in $[0,1]$) of {\MA} on the top ranked answer candidate to weight the loss term for {\MG} corresponding to that instance (question $q$). For a batch of questions $\mathcal{B}{=}\{(q_1,C_1),\dots,(q_m,C_m)\}$, the AS2-score weighted loss function can be presented as follows:

\begin{equation*}
    \mathcal{L}(\mathcal{B}){=}-\frac{1}{m} \sum_{i=0}^{m} w_i \cdot \mathcal{P}\Big(\mathcal{M}_G(q_i,\bar{c})=c^{M_A}_{1}\Big)
\end{equation*}
where $w_i=\mathcal{M}_A\big(q_i,c^{M_A}_{1}\big)$ is the prediction score of {\MA} for the top ranked answer candidate for $q_i$, and  $\mathcal{P}(\cdot)$ is the probability of prediction of the target answer by {\MG} given the input question and $k$ answer candidates as context. In practice, $\mathcal{P}$ is implemented as the log probability of prediction of each token of the target given previous tokens. For the rest of the paper, we will denote the AS2-score loss weighting for training GenQA as {\LW}.


\subsection{AS2 Score Conditioned I/O Shaping}
\label{ssec:SIOLF}

In the previous section, we proposed a method for incorporating the AS2 prediction score for weighting the training loss for GenQA. Alternately, the AS2 prediction score can be incorporated more implicitly for influencing the generation of the GenQA model {\MG}. This is done by means of manipulating the inputs and outputs when training the GenQA model based on the AS2 prediction score. For seq2seq transformer-based text generation models, this is closely related with incorporating and manipulating prompts for the input/output.

We define a bucketing function $\mathcal{F}$ that operates on the AS2 prediction score $\mathcal{M}_A(q,a)$ for a QA pair $(q,a)$ and assigns a confidence bucket $B{=}[b_1,\dots,b_l]$ over the normalized interval $[0,1]$. Here $\mathcal{F}\big(\mathcal{M}_A(q,a)\big)$ is assigned $b_i$ if $\mathcal{M}_A(q,a) \in \Big[\frac{i-1}{l},\frac{i}{l}\Big)$. For our experiments, we set the value of $l{=}5$, and assign a text token for each bucket $b_i \in B$ which correlates with the confidence of the bin in natural text as follows: [`yes',`probably',`maybe',`doubt',`no']. We incorporate  $\mathcal{F}$ for manipulating the input and output of the GenQA model as follows:

\begin{itemize}
    \item \textbf{AS2 Score Conditioned Input:} For each of the $k$ answer candidates to be provided as input $\bar{c}{=}\{c^{M_A}_{2},\dots, c^{M_A}_{k+1}\}$, we assign the natural text token corresponding to the bucket $b_i$ they fall in as per $\mathcal{F}$. We denote the resulting set of text tokens for $\bar{c}$ to be [$I_2,\dots,I_{k+1}$]. We modify the input to the GenQA model to be: ``$q$ [SEP] $I_2 \ c^{M_A}_{2}$ [SEP] $\dots$ [SEP] $I_{k+1} \ c^{M_A}_{k+1}$'', where each answer candidate is prefixed with the confidence bucket token. We denote this by {\SCI}.     
    \item \textbf{AS2 Score Conditioned Output:} For the target answer candidate $c^{M_A}_{1}$, we assign the natural text token corresponding to the bucket $b_i$ it falls in as per $\mathcal{F}$, which we denote by $I_1$. We modify the output target of the GenQA model to be: ``$I_1 \ c^{M_A}_{1}$'', where the target answer is prefixed with the confidence bucket token. We denote this by {\SCO}. 
\end{itemize}

{\SCI} and {\SCO} can be used independently as well as jointly for training the GenQA model {\MG} using {\MA}. {\SCO} is related to {\LW} presented in Sec~\ref{ssec:lossweighting}, but differs in explicitly forcing the generation of {\MG} to be influenced by the confidence score of {\MA}. Using {\SCO} for training {\MG} leads to the generated text starting with one of the confidence bin tokens. During inference, this can be used to estimate the confidence of {\MG} in predicted the generated answer. Furthermore, we can exploit this to control the prediction behavior of {\MG} by forcing the decoding to start from one of these special confidence bin tokens. We explore this empirically in Sec~\ref{sec:experiments}.

==> bak/experiments_Apr22_bak.tex <==
In this section, we first describe the datasets used for our experiments, then the experimental setup and finally we present results.

\subsection{Datasets}
\label{ssec:datasets}

We now present the details of the datasets that we have used for training and evaluating the GenQA model by transferring knowledge from an AS2 model. For training our model, we use large scale unlabeled datasets -- a public dataset with $\sim$800K questions and a larger industrial dataset of $\sim$50M. When available, we finetune on labeled data sources with and without a transfer step. For evaluation, we use test sets from 3 popular public and 1 industrial datasets.

\subsubsection{Unlabeled Data}
\mypara{MS-MARCO Question Answering}~\cite{bajaj2018ms} is a popular machine reading dataset in QA which is often used for NLP tasks like passage ranking, document ranking, and machine reading. We use the training split of MS-MARCO v2.1~\footnote{\url{https://huggingface.co/datasets/ms_marco}} which contains $\sim$800k unique anonymized real user queries from the Bing search engine along with $\sim10$ passages retrieved for each question on average. We split the original dataset into individual sentences using the BlingFire tokenizer\footnote{https://github.com/microsoft/BlingFire} to be used as answer candidates for the AS2 model. We use this data as unlabeled $(q,a)$ pairs for transferring knowledge from \MA to \MG. 

\mypara{WQA-U} is a large scale internal industrial QA dataset containing non-representative de-identified user questions from a commercial virtual assistant. WQA-U contains $\sim$ 50 million questions, and $\sim$ 400 answer candidates retrieved for each question using a large scale web index that contains over 100M web documents. The answer candidates in WQA-U are without any human annotations of correctness/incorrectness. 

\subsubsection{Labeled Data}

\mypara{MS-MARCO NLG} provides at least one manually generated answer for each question from a subset of MS MARCO Question Answering. The train split contains $\sim$ 150k (q,a) pairs.  We sub-sample 1k questions from the development set, along with their answer candidates extracted from the associated passages, to be used for evaluation in our experiments (note that we do not use the entire development set of $\sim$ 100k questions for evaluation due to the expensive cost of human annotations). For complete details and data statistics, refer to Appendix.

\mypara{WQA-L} is the labeled counterpart to the industrial dataset WQA-U defined above, where answer candidates have human annotations of correctness/incorrectness. We split WQA-L into a training and test set each having $\sim$ 50k and $\sim$ 5k questions respectively.  Results on WQA-L are presented relative to the baseline AS2 model due to the data being internal. For complete details and data statistics, refer Appendix.

%\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark that is used for evaluating AS2 models. TREC-QA contains 1226, 82 and 95 questions in it's training, development and test set respectively. For our experiments, we follow the most popular practice of using the `clean' version of TREC-QA where we only retain questions that have at least one positive and one negative answer candidate. This results in the train/development/test sets of TREC-QA having 1226/69/68 questions respectively. 

\mypara{TREC-QA}~\cite{wang2007jeopardy} is a popular QA benchmark used to evaluate AS2 models. For our experiments, we use the filtering and splits proposed in \cite{trecqazeyu}, where all questions have at least one positive and one negative candidate and the test split is larger. The resulting dataset is composed by 816, 204, 340 unique questions respectively for train, development and test set.

\input{Tables/wqa_results}

\mypara{WikiQA}~\cite{yangetal2015wikiqa} is another popular AS2 dataset containing questions from Bing search logs and answer candidates from Wikipedia. We use the most popular setting of retaining questions with at least one positive answer candidate in the train and validation splits, and retaining questions with at least one positive and one negative answer candidate in the test split. This results in train/development/test sets of WikiQA having 2118/296/236 questions respectively.

\subsection{Models and Baselines}
For {\MG} models, we use the base and large versions of T5~\cite{raffeletall2020}. We train these two models on two different splits of MS-MARCO: we used the MS-MARCO NLG trainset for the GenQA model, and the MS-MARCO QA training set for our weak supervised models. For the AS2 model, we use the RoBERTa-Large model trained on ASNQ~\cite{garg2020tanda} as the trained teacher model for MS-MARCO and an ELECTRA-Base model \cite{clark2020electra} trained using the TANDA approach~\cite{garg2020tanda} on the training split of WQA-L as the trained teacher model for WQA-U.

For baselines, we use the RoBERTa-Large models trained using TANDA~\cite{garg2020tanda} on WikiQA and TREC-QA for evaluation. We use the GenQA approach from ~\citet{hsu2021answer} trained on labeled data as the upper bound baseline for our weak supervision GenQA training using the AS2 models.

\subsection{Evaluation and Metrics}
We perform human evaluation of our generated answers using MTurk annotators. We use accuracy as the primary metric for all our experiments and models. This is computed as the average \todo{micro-average instead of majority voting, since the latter one provided unreliable performance.} number of questions a model answers correctly as judged by the annotators. For the AS2 model, the accuracy is the same as Precision@1 which is the precision of the top ranked answer candidate by the AS2 model. 

\subsection{Experimental Details}
\label{ssec:experimental_details}

For our experiments, we set the value of $k$, i.e, the number of answer candidates to be provided as input context to the GenQA model, to be 4. 

We train our models using $fp16$ precision, Adam \cite{Kingma2015AdamAM} as optimizer with a $lr=1e-04$ and a batch size of $256$. We trained each model for $25$ epochs on both the versions of MS-MARCO and for $50$ epochs on WikiQA and TrecQA. We select the best model by maximizing the average AS2 score on the development set of each dataset instead of minimizing the validation loss (see the details in Appendix \ref{apx:ckpt_selection}).

We perform experiments on three different settings:
\subsubsection{MS-MARCO \& MS-MARCO NLG}
With this experiment we train and evaluate our model on a well-known and large dataset. Specifically, this experiment is useful to properly understand the effectiveness of our week supervised methods and to compare them with the original supervised GenQA model. We train our models considering the unlabeled MS-MARCO dataset described in Sec.~\ref{ssec:datasets} and we use a AS2 teacher based on RoBERTa-large and trained on ASNQ for the knowledge transfer. It is important to notice that in this setting, during the training both the student and the teacher model have not any knowledge about the original labels of MS-MARCO. In contrast, the proposed baseline based on the original GenQA model \cite{hsu2021answer} is trained on MS-MARCO NLG which is labeled and also provides high quality manually generated answers. In addition, we propose a two stages training to understand if a second training on a supervised dataset could improve the performance of model trained using our weak supervision techniques. All the models are then evaluated by manual annotators on the same MS-MARCO NLG testset described in Sec.~\ref{ssec:datasets} and the results are reported in terms of accuracy.

\subsubsection{WikiQA \& TrecQA}
In this experiment, we measure the quality of our training approaches evaluating their performance on two AS2 benchmark datasets which are WikiQA and TrecQA. With this setting we explored the capability of the models by answering different research questions. Specifically, we compare our approaches with a strong AS2 baseline and a GenQA model directly trained on this dataset, to verify two hypothesis: first, our approaches can be easily applied and extended to different datasets, and second that a knowledge tranfer from an in-domain teacher could improve the performance of the teacher itself. In addition, we explore further the limitations of the traditional GenQA approach on a few data setting. To perform these experiment, we trained our approaches on a weak supervised setting using MS-MARCO and an AS2 teacher trained directly on TrecQA and WikiQA. In contrast, for the GenQA and the AS2 baseline models, we directly perform the training on the benchmarks. The models were respectively evaluated on the two test splits defined in Sec.~\ref{ssec:datasets}.


%\textcolor{red}{why this experiments?}
%\begin{itemize}
%    \item \textcolor{red}{in this setting we consider smaller datasets}
%    \item \textcolor{red}{our models have some knowledge about them (the as2 teacher model is trained on them)}
%    \item \textcolor{red}{these models does not provide manually generated answers}
%    \item \textcolor{red}{our model trained on more but unlabeled data}
%    \item \textcolor{red}{our model are improving the teacher?}
%\end{itemize}

%\textcolor{red}{setting?}
%\begin{itemize}
%    \item \textcolor{red}{our models are trained on msmarco but having a teacher finetuned on the two considered datasets (wikiqa and trecqa)}
%    \item \textcolor{red}{the hsuetall model is trained directly on the two datasets, and since the dataset have not manually generated answers, during the training we consider as target a positive answer randomly selected from the %original set of candidates}
%    \item \textcolor{red}{the teacher is an AS2 model based on roberta-large and trained directly on the two datasets.}
%    \item 
%\end{itemize}

\subsubsection{Industrial Setting: WQA}

%We perform experiments for two settings: one using publicly available datasets and one on large-scale industrial datasets. For the former, we use the MS-MARCO training split (unlabeled data) for transferring knowledge from the trained AS2 model to train a GenQA model {\MG}. We perform this training using our approach as defined in Sec~\ref{ssec:training_genqa} along with modifications such as {\LW}, {\SCI} and {\SCO}. We evaluate the trained GenQA models on the test split of MS-MARCO and on the test splits of WikiQA and TREC-QA, the latter two corresponding to a zero-shot evaluation. We also perform a second stage of training/fine-tuning following the transfer-then-adapt strategy presented by ~\citet{garg2020tanda} on the training splits of WikiQA and TREC-QA and evaluate the resulting GenQA models on the respective test splits.

For the industrial dataset setting, we use WQA-U for training the GenQA model from the knowledge of the AS2 model. We evaluate the trained GenQA model on the test split of WQA-L. We also perform a second stage fine-tuning on the train split of WQA-L following ~\citet{garg2020tanda} and evaluate the resulting GenQA model on the test split of WQA-L.

\subsection{Results}
In this section we present the results obtained on the three different settings defined in Sec.~\ref{ssec:experimental_details}.

\label{ssec:Results}

\subsubsection{MS-MARCO}
\label{sssec:msmarco_results}
\input{Tables/msmarco_results}

We present the results on the MS-MARCO NLG testset in Table~\ref{tab:msmarco_results} in terms of accuracy. The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points, which is the model with the lowest accuracy in this setting. Our transfer techniques improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with in weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point showing that our seq2seq QA models are robuster and have better generalization capabilities. In addition, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($\text{TL}_{\text{LW+SCI\&SCO}}$) by several accuracy points (0.837 vs 0.853).

%\begin{itemize}
%    \item \textcolor{red}{The AS2 baseline is the model with the lowest results, show that our generative models are robuster and present better generalization capabilities.}
%    \item \textcolor{red}{The original GenQA model trained on the labeled MS-MARCO NLG dataset, outperforms the AS2 baseline by 3.3 accuracy points. }
%    \item \textcolor{red}{Our transfer technique improved both the AS2 and the GenQA baselines. Specifically, the results show that the \textbf{TL} alone obtain comparable performance with the AS2 model but trained with an weak supervision manner. In addition, the LW and SCI\&SCO improve the quality of the knowledge transfer and their combination also outperform the GenQA baseline by 1 accuracy point.}
%    \item \textcolor{red}{Lastly, we noticed that the weak supervision and the supervised GenQA could be also combined in a two stages training outperforming the second best approach ($TL_{LW+SCI\&SCO}$) by several accuracy points (0.837 vs 0.853)}
%\end{itemize}


\subsubsection{WikiQA \& TrecQA}
\label{sssec:qa_results}
\input{Tables/wikiqa_and_trecqa_results}

The results presented in Table \ref{tab:wikiqa_results} and Table \ref{tab:trecqa_results} show that our Transfer Learning techniques have better performance than both the AS2 model and the GenQA baselines. Indeed, we verified the hypothesis that applying our transfer learning techniques can improve the original AS2 model used as a teacher. For examples, in both the datasets our TL model outperform the AS2 baseline by $0.04$ and $4.6$ accuracy points respectively for WikiQA and TrecQA. In addition, we proved that the original GenQA approach requires a bigger dataset to converge to a good solution and to effectively outperform the AS2 models (as we experienced in Sec.\ref{sssec:msmarco_results}).

%\todo{to write this section.}
%\begin{itemize}
%\item \textcolor{red}{TL techniques have better performance then the as2 model. Indeed, we verified the hypotesis that applying these transfer learning techniques can improve the original AS2 model used as a teacher.}
%\item \textcolor{red}{GenQA have poor performance, we can infer that this training setting requires more data to converge to a good solution.}
%\end{itemize}


\subsubsection{Industrial dataset}
\label{sssec:industrial_results}

For the industrial data setting, we present the results in Table~\ref{tab:wqa_results}. Due to the dataset being internal, we only present results relative to the AS2 baseline which is used as the `teacher' for transferring knowledge to train the GenQA model. When using T5-Base as the GenQA model, our results show that knowledge transfer from the AS2 model using the unlabeled data can surprisingly improve the accuracy of the baseline by 2.16\%. This indicates that the weak supervision provided by the AS2 model is able to train a GenQA model that performs better than the AS2 model itself. Furthermore, using loss weighting ({\LW}) and output shaping ({\SCO}) can provide significant improvements to our weak supervision approach. The T5-Base model trained using a combination of the unlabeled and labeled data along with {\LW} and {\SCO} can achieve an impressive 11.8\% gain in accuracy over the baseline AS2 model. We observe a similar trend in results for T5-Large model as well where using the weak supervision from the AS2 model and {\LW} and {\SCO} can provide significant accuracy improvements over the AS2 baseline. 

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|} 
%         \hline
%         Model & Approach & Average Accuracy\% (+-stdev)  \\
%         \toprule
%         human-generated & -- & -- \\
%         roberta-large-tanda-asnq-msmarco & AS2 & -- (+- --) \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-base & GenQA & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW & -- (+- --)\\ 
%         T5UQA-base & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-base & GenQA + LW + SOLF & -- (+- --)\\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- (+- --)\\ 
%         T5UQA-large & GenQA & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW & -- (+- --)\\ 
%         T5UQA-large & GenQA + SOLF & -- (+- --)\\ 
%         T5UQA-large & GenQA + LW + SOLF & -- (+- --)\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the MSMARCO testset.}
%     \label{tab:msmarco_results}
% \end{center}
% \end{table*}

% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with a zero-shot setting. All the GenQA models are trained only on MSMARCO and then evaluated on WikiQA and TrecQA.}
%     \label{tab:wikiqa_zeroshot_results}
% \end{center}
% \end{table*}


% \begin{table*}
% \small
% \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset without labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in Section \ref{sec:genqa_from_as2}}
%     \label{tab:wikiqa_ftu_results}
% \end{center}
% \end{table*}

% \begin{table*}
%     \small
%     \begin{center}
%     \begin{tabular}{|l|c|c|c|} 
%         \hline
%         Model & Approach & WikiQA Acc\% & TrecQA Acc\% \\
%         \toprule
%         roberta-large-tanda-asnq-wikiqa & AS2 & -- & -- \\
%         \midrule
%         T5UQA-base-hsuetall2021 & GenQA Labeled & -- & --\\ 
%         T5UQA-base & GenQA & -- & -- \\ 
%         T5UQA-base & GenQA + LW & -- & -- \\ 
%         T5UQA-base & GenQA + SOLF & -- & -- \\ 
%         T5UQA-base & GenQA + LW + SOLF & -- & -- \\
%         \midrule
%         T5UQA-large-hsuetall2021 & GenQA Labeled & -- & -- \\ 
%         T5UQA-large & GenQA & -- & -- \\ 
%         T5UQA-large & GenQA + LW & -- & -- \\ 
%         T5UQA-large & GenQA + SOLF & -- & -- \\ 
%         T5UQA-large & GenQA + LW + SOLF & -- & --\\ 
%         \hline
%     \end{tabular}
%     \caption{Results on the WikiQA and TrecQA testset with labels supervision. All the GenQA models are trained on MSMARCO and then finetuned on WikiQA and TrecQA using the methods described in \cite{hsu2021answer}.}
%     \label{tab:wikiqa_ftl_results}    
%     \end{center}
% \end{table*}

==> bak/introduction_bak.tex <==
Answering questions by extracting answers from the web, while effective, comes with certain drawbacks. A single web sentence may not contain all information needed to answer a question, or may provide extraneous information unrelated to the information needs of the questioner. Being written for an entirely different purpose, web sentences might be unsuitable as answers due to style issues such as sentiment or formality, or may be structurally reliant on longer discourse context and thus awkward as standalone answers. 

In light of this, researchers have experimented with using text generation systems to answer questions (GenQA). Such generative systems often learn to extract answers from relevant paragraphs~\cite{lewis-etal-2020-bart} or to summarize and synthesize information from the top candidates of an answer sentence selection (AS2) system~\cite{hsu2021answer}. Initial results have shown improvements in terms of both answer accuracy and style suitability. Recent work has extended these techniques to multilingual domains with impressive results~\cite{DBLP:journals/corr/abs-2110-07150}. 

However, a problem for generative QA models is the difficulty of obtaining training data. Existing datasets offer limited coverage of all domains where GenQA can be applied~\cite{bajaj2018ms}, or are too small to use as training data~\cite{DBLP:journals/corr/abs-2110-07150}. Generally, collecting human-authored answers to questions given a context is significantly more expensive compared to annotating the correctness of web sentences as answers. Accordingly, there are more resources available of the latter type~\cite{wang2007jeopardy,yang2015wikiqa,garg2020tanda}. 
 
We propose to transfer the knowledge learned by an AS2 model to a generative QA system. Towards this, we learn an answer generation model using weak supervision provided by a trained AS2 model on a set of unlabeled data. Specifically, the AS2 model is used to generate a ranking over the answer candidates for each question. The top answer is used as the target, while the concatenation of the question and the next 4 top ranked answers is used as the input for the GenQA model. 

In addition to using the weak supervision from the ranking of answers provided by the AS2 model, we also exploit the prediction score for the top answer from the AS2 model by proposing 2 modifications of our training strategy. The first one weighs the training loss of each instance with the score of the top ranked answer from the AS2 model so as to selectively learn more from `good' quality answers. The second manipulates the inputs and outputs to the GenQA model by prefixing the answer candidates with a text token that corresponds to the confidence bin of their AS2 score. 

We perform empirical evaluation on three popular public: MS-MARCO, WikiQA, TREC-QA; and one large scale industrial QA dataset. Our results show that the GenQA model trained using our paradigm of weak supervision from an AS2 model can surprisingly outperform the latter. The answers provided by our GenQA model are often more directly related to the question being asked and stylistically more suitable as responses.
